Towards Mitigating API Hallucination in Code Generated by LLMs with Hierarchical Dependency Aware

Application Programming Interfaces (APIs) are crucial in modern software development. Large Language Models (LLMs) assist in automated code generation but often struggle with API hallucination, including invoking non-existent APIs and misusing existing ones in practical development scenarios. Existing studies resort to Retrieval-Augmented Generation (RAG) methods for mitigating the hallucination issue, but tend to fail since they generally ignore the structural dependencies in practical projects and do not indeed validate whether the generated APIs are available or not. To address these limitations, we propose MARIN, a framework for mitigating API hallucination in code generated by LLMs with hierarchical dependency aware. MARIN consists of two phases: Hierarchical Dependency Mining, which analyzes local and global dependencies of the current function, aiming to supplement comprehensive project context in LLMs input, and Dependency Constrained Decoding, which utilizes mined dependencies to adaptively constrain the generation process, aiming to ensure the generated APIs align with the projects specifications. To facilitate the evaluation of the degree of API hallucination, we introduce a new benchmark APIHulBench and two new metrics including Micro Hallucination Number (MiHN) and Macro Hallucination Rate (MaHR). Experiments on six state-of-the-art LLMs demonstrate that MARIN effectively reduces API hallucinations, achieving an average decrease of 67.52% in MiHN and 73.56% in MaHR compared to the RAG approach. Applied to Huaweis internal projects and two proprietary LLMs, MARIN achieves average decreases of 57.33% in MiHN and 59.41% in MaHR.

==> FSE25-Industry-APIMitigation_2/datas/RQ1_table.tex <==
% Please add the following required packages to y{\tool} document preamble:
% \usepackage{multirow}
% \begin{table*}
% \caption{xxx}
% \begin{tabular}{c|c|ccccc|ccccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Approach}} & \multicolumn{5}{c|}{{\dataset}-F} & \multicolumn{5}{c}{{\dataset}-M} \\ \cline{3-12} 
%  &  & EM(\%) & ES(\%) & IM(\%) &  MaHR(\%) & MiHN & EM(\%) & ES(\%) & IM(\%) &  MaHR(\%) & MiHN  \\ \midrule
% \multirow{4}{*}{CodeLlama-7B} & Base & 21.71 & 46.32 & 28.95 & 73.30 & 0.79 & 27.69 & 55.69 & 35.89 & 65.12 & 0.74 \\
%  & RAG & 27.60 & 50.71 & 34.84 & 67.87 & 0.71 & 36.41 & 61.10 & 47.69 & 53.84 & 0.61 \\
%  & De-Hallucinator & 22.17 & 46.79 & 29.41  & 73.30 & 0.81 & 29.89  & 56.62 & 40.20 &60.30  &  0.71 \\
%  & {\tool} & 76.01 & 87.04 & 87.33 & 15.83  & 0.17  & 66.66 & 83.66 & 89.23 & 12.30 & 0.13 \\ \midrule
% \multirow{4}{*}{CodeLlama-13B} & Base & 33.03 & 60.05 & 39.81 & 61.08 & 0.71 & 33.33 & 61.73 & 41.02 & 59.48 & 0.70 \\
%  & RAG & 49.32 & 69.78 & 59.27 & 42.98 & 0.48 & 36.41  & 61.61 & 48.71 & 52.82 &  0.61 \\
%  & De-Hallucinator & 41.62 & 66.35 & 49.32 & 52.03 & 0.60 & 32.98 & 62.24 & 41.75 & 58.76 & 0.69 \\
%  & {\tool} & 66.96 & 80.20 & 74.20 & 28.95  & 0.33  & 66.66 & 84.09 & 88.20 & 12.30 & 0.13 \\ \midrule
% \multirow{4}{*}{CodeLlama-34B} & Base & 19.45 & 51.62 & 27.14 & 75.56 & 0.81 & 24.61 & 55.02 & 32.30 & 68.71 & 0.74 \\
%  & RAG & 31.67 & 55.21 & 39.36 & 63.80 & 0.66 & 38.46  & 62.59 & 48.20 & 52.82  & 0.58 \\
%  & De-Hallucinator & 18.09 & 49.25 &25.79  & 76.47 & 0.84 & 26.28 & 55.50 & 33.50 & 67.52 & 0.76 \\
%  & {\tool} & 81.90 & 89.75 & 90.49 & 12.66 & 0.13 & 70.76 & 86.24 & 90.76  & 10.76 &  0.12 \\ \midrule
% \multirow{4}{*}{DeepSeekCoder-1.3B} & Base & 21.71 & 52.19 & 29.41 & 72.85 & 0.87 & 23.58 & 52.71 & 32.82 & 68.20 & 0.82 \\
%  & RAG & 38.91 & 63.04 & 46.15 & 56.10 & 0.67 & 34.87 & 61.26 & 44.61 & 56.41 & 0.71 \\
%  & De-Hallucinator & 40.27 & 64.81 & 46.60 & 54.29 & 0.63 & 30.92 & 57.06 & 40.20 & 60.30 & 0.71 \\
%  & {\tool} & 75.11 & 86.82 & 84.61 & 17.64 & 0.19 & 64.61 & 82.34 & 85.64 & 15.38 & 0.16 \\ \midrule
% \multirow{4}{*}{DeepSeekCoder-6.7B} & Base & 20.81 & 49.00 & 25.33 & 75.56 & 0.82 & 23.07  & 51.78 & 31.28 & 68.71 &  0.76 \\
%  & RAG & 37.10  & 59.57 & 42.98 & 57.46 & 0.64 & 33.33 & 58.90 & 44.10 & 56.92 & 0.65 \\
%  & De-Hallucinator & 31.22 & 56.88 & 39.36 & 64.25 &  0.72 & 24.22 & 53.39 & 32.47 & 67.52 & 0.77 \\
%  & {\tool} & 75.56 & 87.65 & 86.42 & 16.74 &  0.18 & 68.20 & 85.23 & 89.74 & 11.28 & 0.11 \\ \midrule
% \multirow{4}{*}{DeepSeekCoder-33B} & Base & 35.74 & 57.99 & 41.62 & 59.72 & 0.66 & 20.00 & 51.98 & 30.25 & 70.25 & 0.78 \\
%  & RAG & 46.15 & 67.40 & 54.29 & 47.05 & 0.50 & 36.41 &  61.90 & 46.15 & 54.35 & 0.60 \\
%  & De-Hallucinator & 42.98 & 64.45 & 48.86 & 52.03 & 0.57 & 27.83 & 57.26 & 36.59 & 63.40  & 0.71 \\
%  & {\tool} & 81.90 & 90.83 & 91.40 & 11.76 & 0.13 & 67.69 & 85.39 & 91.28 & 9.74 & 0.10 \\ \bottomrule
% \end{tabular}
% \end{table*}
% 请确保在导言区添加以下包：
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{xcolor}
\begin{table*}[t]
 % \renewcommand{\arraystretch}{0.95} % 默认值是 1
 % \setlength{\abovecaptionskip}{-1pt} 
\caption{Evaluation results of baseline approaches and {\tool} on two benchmarks, \textbf{\raisebox{0.5ex}{\textasteriskcentered}} denotes statistically significant improvement (t-test with p-value < 0.001) over the baseline approaches.}
\label{Table:res_main}
\begin{tabular}{c|c|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Approach}} & \multicolumn{5}{c|}{\textbf{{\dataset}-F}} & \multicolumn{5}{c}{\textbf{{\dataset}-M}} \\ \cline{3-12} 
 &  & EM(\%) & ES(\%) & IM(\%) & MaHR(\%) & MiHN & EM(\%) & ES(\%) & IM(\%) & MaHR(\%) & MiHN  \\ \midrule
\multirow{4}{*}{CodeLlama-7B} & Base & 21.71 & 46.32 & 28.95 & 73.30 & 0.79 & 27.69 & 55.69 & 35.89 & 65.12 & 0.74 \\
 & RAG & 27.60 & 50.71 & 34.84 & 67.87 & 0.71 & 36.41 & 61.10 & 47.69 & 53.84 & 0.61 \\
 & De-Hallucinator & 22.17 & 46.79 & 29.41  & 73.30 & 0.81 & 29.89  & 56.62 & 40.20 &60.30  &  0.71 \\
& {\cellcolor{gray!20}\textbf{\tool}} & {\cellcolor{gray!20}\textbf{76.01\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{87.04\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{87.33\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{15.83\raisebox{0.5ex}{\textasteriskcentered}}}  & {\cellcolor{gray!20}\textbf{0.17\raisebox{0.5ex}{\textasteriskcentered}}}  & {\cellcolor{gray!20}\textbf{66.66\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{83.66\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{89.23\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{12.30\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.13\raisebox{0.5ex}{\textasteriskcentered}}} \\ \midrule
\multirow{4}{*}{CodeLlama-13B} & Base & 33.03 & 60.05 & 39.81 & 61.08 & 0.71 & 33.33 & 61.73 & 41.02 & 59.48 & 0.70 \\
 & RAG & 49.32 & 69.78 & 59.27 & 42.98 & 0.48 & 36.41  & 61.61 & 48.71 & 52.82 &  0.61 \\
 & De-Hallucinator & 41.62 & 66.35 & 49.32 & 52.03 & 0.60 & 32.98 & 62.24 & 41.75 & 58.76 & 0.69 \\
& {\cellcolor{gray!20}\textbf{\tool}} & {\cellcolor{gray!20}\textbf{66.96\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{80.20\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{74.20\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{28.95\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.33\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{66.66\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{84.09\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{88.20\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{12.30\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.13\raisebox{0.5ex}{\textasteriskcentered}}} \\ \midrule
\multirow{4}{*}{CodeLlama-34B} & Base & 19.45 & 51.62 & 27.14 & 75.56 & 0.81 & 24.61 & 55.02 & 32.30 & 68.71 & 0.74 \\
 & RAG & 31.67 & 55.21 & 39.36 & 63.80 & 0.66 & 38.46  & 62.59 & 48.20 & 52.82  & 0.58 \\
 & De-Hallucinator & 18.09 & 49.25 &25.79  & 76.47 & 0.84 & 26.28 & 55.50 & 33.50 & 67.52 & 0.76 \\
& {\cellcolor{gray!20}\textbf{\tool}} & {\cellcolor{gray!20}\textbf{81.90\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{89.75\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{90.49\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{12.66\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.13\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{70.76\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{86.24\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{90.76\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{10.76\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.12\raisebox{0.5ex}{\textasteriskcentered}}} \\ \midrule
\multirow{4}{*}{DeepSeekCoder-1.3B} & Base & 21.71 & 52.19 & 29.41 & 72.85 & 0.87 & 23.58 & 52.71 & 32.82 & 68.20 & 0.82 \\
 & RAG & 38.91 & 63.04 & 46.15 & 56.10 & 0.67 & 34.87 & 61.26 & 44.61 & 56.41 & 0.71 \\
 & De-Hallucinator & 40.27 & 64.81 & 46.60 & 54.29 & 0.63 & 30.92 & 57.06 & 40.20 & 60.30 & 0.71 \\
& {\cellcolor{gray!20}\textbf{\tool}} & {\cellcolor{gray!20}\textbf{75.11\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{86.82\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{84.61\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{17.64\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.19\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{64.61\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{82.34\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{85.64\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{15.38\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.16\raisebox{0.5ex}{\textasteriskcentered}}} \\ \midrule
\multirow{4}{*}{DeepSeekCoder-6.7B} & Base & 20.81 & 49.00 & 25.33 & 75.56 & 0.82 & 23.07  & 51.78 & 31.28 & 68.71 &  0.76 \\
 & RAG & 37.10  & 59.57 & 42.98 & 57.46 & 0.64 & 33.33 & 58.90 & 44.10 & 56.92 & 0.65 \\
 & De-Hallucinator & 31.22 & 56.88 & 39.36 & 64.25 &  0.72 & 24.22 & 53.39 & 32.47 & 67.52 & 0.77 \\
& {\cellcolor{gray!20}\textbf{\tool}} & {\cellcolor{gray!20}\textbf{75.56\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{87.65\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{86.42\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{16.74\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.18\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{68.20\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{85.23\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{89.74\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{11.28\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.11\raisebox{0.5ex}{\textasteriskcentered}}} \\ \midrule
\multirow{4}{*}{DeepSeekCoder-33B} & Base & 35.74 & 57.99 & 41.62 & 59.72 & 0.66 & 20.00 & 51.98 & 30.25 & 70.25 & 0.78 \\
 & RAG & 46.15 & 67.40 & 54.29 & 47.05 & 0.50 & 36.41 &  61.90 & 46.15 & 54.35 & 0.60 \\
 & De-Hallucinator & 42.98 & 64.45 & 48.86 & 52.03 & 0.57 & 27.83 & 57.26 & 36.59 & 63.40  & 0.71 \\
& {\cellcolor{gray!20}\textbf{\tool}} & {\cellcolor{gray!20}\textbf{81.90\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{90.83\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{91.40\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{11.76\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.13\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{67.69\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{85.39\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{91.28\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{9.74\raisebox{0.5ex}{\textasteriskcentered}}} & {\cellcolor{gray!20}\textbf{0.10\raisebox{0.5ex}{\textasteriskcentered}}} \\ \bottomrule
\end{tabular}
% \begin{tablenotes} 
% \centering
% % \modify{\}
% \end{tablenotes}
\end{table*}

==> FSE25-Industry-APIMitigation_2/datas/RQ3_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}
% \caption{xxx}
% \small
% \begin{tabular}{c|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{Approach} & \multicolumn{6}{c|}{{\dataset}-F}                       & \multicolumn{6}{c}{{\dataset}-M}                        \\ \cline{2-13} 
%                           & CL-7B & CL-13B & CL-34B & DSC-1.3B & DSC-6.7B & DSC-33B & CL-7B & CL-13B & CL-34B & DSC-1.3B & DSC-6.7B & DSC-33B \\ \midrule
% Base                      & 0.228     &  0.203     & 0.379       &   0.214       & 0.217         & 0.309          & 0.216      &  0.204      &  0.380      &   0.209       & 0.211         &   0.319      \\ \midrule
% RAG               & 0.684 &  0.526  & 0.874    & 0.659 &  0.664 & 0.888  &  0.935  & 0.910  &   1.054   &      0.916    &   0.919       & 1.045         \\ \midrule
% De-Hal.           &  0.571     &  0.729     & 0.906   &  0.551       &  0.773      & 0.865           &  0.560   &0.744      & 0.950        & 0.552   &  0.768        & 0.858     \\ \midrule
% {\tool}         & 0.254     &   0.276     &  0.418      &  0.226        &   0.283       &  0.329        &  0.256     &  0.202      & 0.453       &  0.210        &  0.210        & 0.333          \\ \bottomrule
% \end{tabular}
% \end{table*}
\begin{table*}[t]
% \setlength{\abovecaptionskip}{-1pt} 
% \renewcommand{\arraystretch}{0.9} 
\caption{Computational time comparison across baseline approaches and {\tool}. The abbreviation ``De-Hal.'' denotes ``De-Hallucinator'', the ``CL'' denotes ``CodeLlama'' and the ``DSC'' denotes ``DeepSeekCoder''.}
\label{table:res_efficiency}
% \small
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Approach}} & \multicolumn{6}{c|}{\textbf{{\dataset}-F}}                       & \multicolumn{6}{c}{\textbf{{\dataset}-M}}                        \\ \cline{2-13} 
                          & CL-7B & CL-13B & CL-34B & DSC-1.3B & DSC-6.7B & DSC-33B & CL-7B & CL-13B & CL-34B & DSC-1.3B & DSC-6.7B & DSC-33B \\ \midrule
Base                      & 0.203      &  0.228   & 0.379       &   0.214       & 0.217         & 0.309          & 0.204      &  0.216      &  0.380      &   0.209       & 0.211         &   0.319      \\ \midrule
RAG               & 0.526  &  0.684  & 0.874    & 0.659 &  0.664 & 0.888  &  0.910  & 0.935  &   1.054   &      0.916    &   0.919       & 1.045         \\ \midrule
De-Hal.           &  0.571     &  0.729     & 0.906   &  0.551       &  0.773      & 0.865           &  0.560   &0.744      & 0.950        & 0.552   &  0.768        & 0.858     \\ \midrule
\rowcolor{gray!20} % 添加灰色背景
{\textbf{\tool}}         & \textbf{0.214}     &   \textbf{0.276}     &  \textbf{0.418}      &  \textbf{0.226}        &   \textbf{0.233}       &  \textbf{0.329}        &  \textbf{0.216}     &  \textbf{0.232}      & \textbf{0.453}       &  \textbf{0.210}        &  \textbf{0.215}        & \textbf{0.333}          \\ \bottomrule
\end{tabular}
\end{table*}

% 10 并发 for 30B+
% 20 并发 for < 10B+

==> FSE25-Industry-APIMitigation_2/datas/RQ4_table.tex <==

\begin{table}
% \setlength{\abovecaptionskip}{-1pt}
 % \renewcommand{\arraystretch}{0.85} 
\centering
\caption{Evaluation results of baseline approaches and {\tool} in the industry scenario. The abbreviation of ``De-Hal.'' denotes ``De-Hallucinator''. \textbf{\raisebox{0.5ex}{\textasteriskcentered}} denotes statistically significant improvement (t-test with p-value < 0.001) over the baseline approaches.}
\label{table:res_industry}
\small
\begin{tabular}{c|ccccc}
\toprule
\textbf{Approach}                       & \textbf{EM(\%)} & \textbf{ES(\%)} & \textbf{MaHR(\%)} & \textbf{MiHN} & \textbf{Time(s)} \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}PanguCoder-11B}                           \\ \midrule
\multicolumn{1}{c|}{Base}    &  13.63      &  50.53      &   85.45       &  1.06    &   0.205      \\ \midrule
\multicolumn{1}{c|}{RAG}     &  35.45      &   60.97     &       60.90     &   0.73    &  0.411      \\ \midrule
\multicolumn{1}{c|}{De-Hal.} &  13.76      &  48.72      &     86.23  &  1.11  &  0.479     \\ \midrule
\multicolumn{1}{c|}{{\textbf{\tool}}}     &  \textbf{60.90\raisebox{0.5ex}{\textasteriskcentered}}      &  \textbf{80.19\raisebox{0.5ex}{\textasteriskcentered}}      &   \textbf{25.45\raisebox{0.5ex}{\textasteriskcentered}}       &  \textbf{0.31\raisebox{0.5ex}{\textasteriskcentered}}    & \textbf{0.235}        \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}PanguCoder-34B}                           \\ \midrule
\multicolumn{1}{c|}{Base}    & 13.63       &  48.27      &   84.54       &  1.05    &  0.206       \\ \midrule
\multicolumn{1}{c|}{RAG}     & 33.63       &  63.80      &   60.00     &  0.70    &    0.479     \\ \midrule
\multicolumn{1}{c|}{De-Hal.} &   13.76     & 49.80       &  85.32        &  1.04    & 0.501      \\ \midrule
\multicolumn{1}{c|}{{\textbf{\tool}}}     &  \textbf{58.18\raisebox{0.5ex}{\textasteriskcentered}}      &   \textbf{78.21\raisebox{0.5ex}{\textasteriskcentered}}     &   \textbf{23.63\raisebox{0.5ex}{\textasteriskcentered}}       & \textbf{0.30\raisebox{0.5ex}{\textasteriskcentered}}     & \textbf{0.239}        \\ \midrule
\end{tabular}
% \begin{tablenotes} 
% % \centering
% \textbf{\raisebox{0.5ex}{\textasteriskcentered}} denotes statistically significant improvement (t-test with p-value < 0.001) over the baseline approaches.
% \end{tablenotes}
\end{table}

==> FSE25-Industry-APIMitigation_2/datas/benchmark-statistics.tex <==
\begin{table}[]
\centering
\begin{tabular}{lrrrr}
\toprule
\textbf{Benchmark}                 & \textbf{APIHulBench} \\
\midrule
\ Language                        & Java             \\
\# Repositories                  & 244             \\
\# Files                         & 47751           \\
\# Examples                      & 2856           \\
Avg. \# lines in prompt          & 18.34          \\
Avg. \# tokens in prompt         & 145.73           \\
Avg. \# lines in reference       & 1.0             \\
Avg. \# tokens in reference      & 8.18            \\
\bottomrule
\end{tabular}
\caption{APIHulBench statistics.}
\label{tab:crosscodeeval}
\end{table}


==> FSE25-Industry-APIMitigation_2/sections/0_abs.tex <==
Application Programming Interfaces (APIs) are crucial in modern software development. Large Language Models (LLMs) assist in automated code generation but often struggle with API hallucination, including invoking non-existent APIs and misusing existing ones in practical development scenarios. Existing studies resort to Retrieval-Augmented Generation (RAG) methods for mitigating the hallucination issue, but tend to fail since they generally ignore the structural dependencies in practical projects and do not indeed validate whether the generated APIs are available or not. To address these limitations, we propose {\tool}, a framework for mitigating API hallucination in code generated by LLMs with hierarchical dependency aware. {\tool} consists of two phases: \textit{{\phaseone}}, which analyzes local and global dependencies of the current function, aiming to supplement comprehensive project context in LLMs' input, and \textit{{\phasetwo}}, which utilizes mined dependencies to adaptively constrain the generation process, aiming to ensure the generated APIs align with the project's specifications. To facilitate the evaluation of the degree of API hallucination, we introduce a new benchmark {\dataset} and two new metrics including Micro Hallucination Number (MiHN) and Macro Hallucination Rate (MaHR). Experiments on six state-of-the-art LLMs demonstrate that {\tool} effectively reduces API hallucinations, achieving an average decrease of 67.52\% in MiHN and 73.56\% in MaHR compared to the RAG approach. Applied to Huawei's internal projects and two proprietary LLMs, {\tool} achieves average decreases of 57.33\% in MiHN and 59.41\% in MaHR.

% an average exact match of 59.54\%, edit similarity of 79.20\%, MaHR of 24.54\% and MiHN of 0.30. 


% Application Programming Interfaces (APIs) are crucial in modern software development, enabling efficient integration of complex functionalities. Large Language Models (LLMs) have become powerful tools for assisting developers in automated code generation. However, in practical development scenarios, they often struggle with invoking non-existent APIs or misusing existing APIs in the generated code, known as ``API hallucination''. Existing Retrieval-Augmented Generation (RAG) based methods use similar project code and relevant API references as supplementary context to mitigate this issue, but still struggle with a lack of comprehensive project context and insufficient API usage guidance. To address these limitations, we propose {\tool}, a framework for mitigating API hallucination in LLM-generated code via hierarchical dependency. {\tool} consists of two phases: \textit{{\phaseone}} and \textit{{\phasetwo}}. \textit{{\phaseone}} analyzes the project to extract local and global dependencies, aiming at constructing a hierarchical presentation of the project repository. \textit{{\phasetwo}} constrains the LLM's decoding process by dynamically masking the output space to valid API candidates, aiming at guiding the model toward contextually appropriate APIs. These two phases work together to leverage rich project knowledge, supplementing context dependencies externally and intervening in the decoding process internally, thereby reducing API hallucination. To evaluate API hallucination, we introduce {\dataset}, a novel benchmark based on open-source projects, and two new metrics: Micro Hallucination Number (MiHN) and Macro Hallucination Rate (MaHR). We validate the effectiveness of {\tool} on six state-of-the-art LLMs with varying model families and sizes. Experimental results show that {\tool} significantly reduces API hallucinations in LLM-generated code, with an average decrease of 3x in MiHN and a 3x decrease in MaHR. To further validate its effectiveness in the industry, we apply {\tool} to Huawei's internal projects and proprietary LLMs. The results demonstrate that {\tool} can effectively and efficiently mitigate API hallucination, achieving an exact match of xxx\%, an edit similarity of xxx\%, an MiHN of xxx, and an MaHR of xxx\%, without introducing additional latency.


==> FSE25-Industry-APIMitigation_2/sections/1_intro.tex <==

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.3]{figures/fig2(a)3error-types.pdf}
%     \caption{xxxx}
%     \label{fig:intro_type}
% \end{figure}

\begin{figure*}
    \centering
    \includegraphics[scale=0.53]{figures/intro_example.pdf}
    \caption{The motivation example: A Wrong API generated by CodeLLama-7B with RAG.}
    \label{fig:intro_example1}
\end{figure*}

In modern software development, developers frequently leverage application programming interfaces (APIs) to integrate complex functionalities into their projects efficiently~\cite{intro_api,intro_api_2,intro_api_3, DBLP:journals/tse/ChenGRP0L23,DBLP:conf/wcre/ChenGZ0WX24}. The advent of large language models (LLMs) has revolutionized this process, with AI-powered coding assistants greatly enhancing developers' productivity by generating code snippets automatically~\cite{intro_au_1,intro_au_2,intro_productivity_1,intro_productivity_2,intro_productivity_3}. However, despite their impressive capabilities, LLMs still face notable challenges in industrial development scenarios. A recent study evaluating six mainstream LLMs on practical code generation shows that 31.67\% of erroneous code directly results from incorrect API usage, a phenomenon named ``API hallucinations''~\cite{zhang2024llm}, including invoking non-existent APIs, misusing existing APIs, and 
% or 
incorrectly using arguments~\cite{jain2024mitigating}. Such mistakes increase debugging complexity since they can propagate errors in subsequent programming.
% code snippets. 
Moreover, a recent study reports that 29\% of security vulnerabilities in the Linux kernel in 2021 were traced back to improper API usage~\cite{intro-misuseapi}. Given the critical role of APIs in developers' daily workflows and the severe consequences of their misuse, exploring effective mitigation methods has become a critical research focus.
Existing studies primarily rely on Retrieval-Augmented Generation (RAG) techniques~\cite{jain2024mitigating,eghbali2024hallucinator,zhang2024llm}, which first construct the retrieval corpora including API documentation and code snippets from the project, and then integrate the retrieved relevant information into the input prompt.
% libraries of  API documentation or repository code snippets, retrieve relevant information, and integrate the retrieved relevant information into the code generation process. 
While these studies have demonstrated success in mitigating API hallucination, they still face the following limitations. 

\textit{1) Ignoring structural dependencies in projects}. When developers call APIs, they typically rely on the structural dependencies of the current code snippet, such as relationships with other functions and modules, to ensure proper API usage within the project context. However, existing approaches fail to consider these critical dependencies, and instead, they offer isolated code snippets as references for LLMs. As illustrated in Figure~\ref{fig:intro_example1}\textcircled{1}, the incomplete function attempts to determine whether an agent will react, and the correct API to be used is {\tt willReact}. 
However, the retrieved code snippet (Figure~\ref{fig:intro_example1}\textcircled{3}) fails to provide sufficient context from related files (Figure~\ref{fig:intro_example1}\textcircled{2}) where the {\tt willReact} method is defined.
Besides, maintaining a retrieval corpus with updated indexing introduces additional resource costs, limiting the scalability of such approaches. 

\textit{2) Unconstrained API generation.} Existing approaches 
utilize auto-regressive decoding, where tokens are generated solely based on model probabilities without explicit constraints on the output space {of API tokens. This unconstrained process often leads to the generation of invalid API tokens. As demonstrated in Figure~\ref{fig:intro_example1}\textcircled{4}, the model generates candidate API tokens {\tt get}, {\tt Re}, {\tt act}, 
{\tt ())}, which does
% do 
not match the intended API {\tt willReact} defined in the {\tt Reaction} class. Such errors occur because the model lacks constraints to align generated tokens
% token generation 
with the actual project specifications, resulting in incorrect and infeasible API calls. This highlights the need to enforce output validity during the decoding process.
% \modify{
% \textit{1) Lack of project structural information.} Practical projects contain extensive structural and semantic information. Structural information captures complex dependencies between modules and methods, while semantic information describes implementation details in code snippets. Current RAG-based methods primarily utilize semantic information by retrieving relevant code snippets, lacking in exploring important structural dependencies within the project, such as method call relationships for the current function. As demonstrated in Section~\ref{}, incorporating such structural information helps reduce API hallucinations.}

% \modify{
% \textit{2) Lack of generation validation.} Based on the input context, LLMs generate code through an auto-regressive decoding process. Existing RAG-based methods emphasize improving the input by supplying reference information, lacking validation during the decoding process. As a result, the generated code may still include invalid APIs, since the generation space remains unconstrained by project-specific dependencies.}

% \textit{1) Lack of comprehensive project context.} Current RAG-based methods typically utilize only code snippets or API documentation as supplementary information, which fails to capture the full structure of the project, leading to an incomplete understanding of the codebase. Our preliminary study (See Section~\ref{}) demonstrates that providing more comprehensive project information leads to superior performance, even surpassing traditional RAG-based methods.

% \textit{2) Insufficient API usage guidance.} While RAG-based methods attempt to guide model generation by retrieving API references from libraries, our observations suggest that simply providing API information in the prompt is insufficient. As seen in Section~\ref{}, XX\% of generated APIs remain invalidated. This highlights the need for more effective mechanisms to constrain the model's output to contextually appropriate APIs during the code generation process.

\noindent \textbf{Our work.} To address these limitations, in this paper, we propose {\tool}, a framework designed to \textbf{M}itigate \textbf{A}PI hallucination in code gene\textbf{R}ated by LLMs with h\textbf{I}erarchical depe\textbf{N}dency aware. Specifically, {\tool} comprises two phases: \textit{1) {\phaseone}.} This phase uses static analysis to analyze local and global dependencies of the current function, such as method call relationships and file dependencies, forming a structural
% hierarchical 
representation of the project to enrich LLM's input prompt. \textit{2) {\phasetwo.}} This phase adaptively constrains the token generation process using valid API patterns derived from the mined dependencies, ensuring the alignment of generated APIs
% align 
with project specifications. 
% % dynamically masks the output space to validate API candidates using the extracted hierarchical dependencies. It aims to constrain the LLM's decoding process to guide the model toward validated API usage. 
% Through the two phases, {\tool} employs project structural dependencies in the input prompt with constrained decoding, 
Through the two phases, {\tool} employs project structural dependencies both in supplying the input and guiding the generation, eliminating the need for retrieval corpora construction, thus enabling effective API hallucination mitigation in the code generation process of LLMs.

% mines project structural dependencies, incorporating them in the input prompt externally and constraining the decoding process internally,
% utilizes combining them with adaptive decoding constraints internally  to 
% bridge the gap between incomplete context and accurate API usage. 
% % leverages rich project knowledge to supplement 
% hierarchical dependencies externally and constrain the decoding process internally, %together 
% \fgd{thereby} mitigating API hallucination in %the code generated by LLMs.
% \fgd{code generation process of LLMs. }
Existing API hallucination evaluation benchmarks suffer from potential data leakage from older repositories~\cite{eghbali2024hallucinator} or reliance on model-synthesized data~\cite{jain2024mitigating, tian2024codehalu}. Therefore, we introduce {\dataset}, a novel benchmark, comprising 416 high-quality samples from 98 recent Java repositories on GitHub. It encompasses two different coding processes: {\dataset}-F (221 samples) where developers initiate new functions, and {\dataset}-M (195 samples) where developers have written most of the code in functions. For evaluating the degree of API hallucination, we also propose two new metrics: Micro Hallucination Number (MiHN), which quantifies
% quantifying 
the number of hallucinated elements within one generated API, and Macro Hallucination Rate (MaHR), which measures
% measuring 
the proportion of the generated APIs containing hallucinations. We apply {\tool} to six state-of-the-art LLMs with varying architectures and sizes (CodeLlama-7B/13B/34B~\cite{codellama} and DeepSeekCoder-1.3B/6.7B/33B~\cite{deepseek}) using the {\dataset} benchmark.
% benchmarks. 
Experimental results demonstrate that {\tool} can significantly mitigate API hallucination of LLM-generated code, with an average decrease of 67.52\% in MiHN and 73.56\% in MaHR as well as an average increase of 107.3\% in exact match (EM) and 44.79\% in edit similarity (ES) compared to RAG approach. To further validate {\tool}'s effectiveness in industry settings, we construct an additional benchmark comprising 109 samples from Huawei's internal projects and apply {\tool} on Huawei's proprietary LLMs (PanguCoder-11B/34B~\cite{pangucoder}). 
The results indicate that {\tool} effectively and efficiently mitigates API hallucination, achieving an average decrease of 59.41\% in MaHR and an average increase of 72.39\% in EM, with only an average 0.031s overhead increase compared to the base model. We release {\dataset} at \url{https://github.com/yujiachen99/APIMitigation}. 

% \input{datas/pre_figure}
%----------------------------定义颜色----------------------------------
\definecolor{p1}{RGB}{174,223,172} % green
\definecolor{p2}{RGB}{224,175,107}  % orangle
\definecolor{p3}{RGB}{138,170,214}  % light blue
\definecolor{p4}{RGB}{222,117,123} %  % red
\definecolor{p5}{RGB}{216,174,174} % light pink
\definecolor{p6}{RGB}{163,137,214} % purple
\definecolor{p7}{RGB}{248,199,1} %  % yellow
\definecolor{p8}{RGB}{205,205,205} % grey
\definecolor{p9}{RGB}{255,0,127} % purple

%-------------------数据------------------------------
\pgfplotstableread[row sep=\\,col sep=&]{
	datasets & evol & oss \\%改数据
	  2 & 0.1454 & 0.8272\\
        4 & 0.1090 & 0.8454\\
        6 & 0.1272 & 0.8727\\
        8 & 0.1181 & 0.8636\\
}\dskfive

\pgfplotstableread[row sep=\\,col sep=&]{
	datasets & base & RAG & P-C & API-G\\%改数据
	  2 & 0.8272 & 0.7272 & 0.6521 & 0.5636\\
        4 & 0.8454 & 0.7181 & 0.6884 & 0.5289\\
        6 & 0.8727 & 0.7181 & 0.6959 & 0.5818\\
        8 & 0.8636 & 0.7727 & 0.6884 & 0.5727\\
}\dskfive
%---------------


\begin{figure*}[t]
\small
\setlength{\abovecaptionskip}{-2pt} % 调整标题与图片之间的间距
\centering
% \setlength{\belowcaptionskip}{-5pt} % 调整标题与图片之间的间距
% \setlength{\abovecaptionskip}{-0.01cm}
% 左侧的 a 图
\begin{minipage}[t]{0.475\textwidth} % 左侧占 40% 宽度
    \centering
    \subfigure[An illustration example of two types of APIs]{
        \includegraphics[width=\textwidth]{figures/pre-types-2.pdf}
        \label{fig:sub_a}
    }
\end{minipage}
% \hfill
% 右侧的 b 图和 c 图
\begin{minipage}[t]{0.48\textwidth} % 右侧占 58% 宽度
    % \ref{plotsub_a}\\
    \setlength{\abovecaptionskip}{-0.01cm}
    \setlength{\abovecaptionskip}{-25pt} % 调整标题与图片之间的间距
    \centering
    % 右上 b 图
    \subfigure[Hallucination across different API types]{
        \begin{tikzpicture}[scale=0.75]
    \begin{axis}[
        grid=major,
        ybar=0.2pt,
        bar width=0.45cm,
        % enlarge x limits=0.15,
        width=1.2\textwidth,
        height=0.35\textwidth,
        xtick=data,
        xticklabels={CL-7B, CL-13B, DSC-1.3B, DSC-6.7B},
        ymin=0, ymax=1.2,
        legend style={
            legend columns=-1, 
            draw=none, 
            font=\large, 
            at={(0.5,1.1)}, % 将图例放在右侧
            anchor=south,
            inner sep=0pt
        },
        legend image code/.code={
            \draw [#1] (0cm,-0.08cm) rectangle (0.4cm,0.1cm); 
        },
        % legend cell align={left},
        legend image post style={scale=0.9, thick},
        % legend to name = plotsub_a,
        tick align=outside,
        % legend pos=outer northeast,
        xticklabel style={font=\normalsize},
        yticklabel style={font=\large},
        every axis plot/.append style={line width=1pt},
        every axis/.append style={line width=1pt},
        ylabel={\textbf{\large MaHR}}, 
        ticklabel style={font=\normalsize},
        nodes near coords,
        nodes near coords style={font=\large,xshift=-4pt}
    ]
    \addplot[fill=p7] table[x=datasets, y=evol]{\dskfive};
    \addplot[fill=p6] table[x=datasets, y=oss]{\dskfive};
    \legend{{\normalem Third-party APIs}, {\normalem Project-specific APIs}};
    \end{axis}
        \end{tikzpicture}
        \label{fig:sub_b}       
        \setlength{\belowcaptionskip}{-25pt} % 调整标题与图片之间的间距
    }
    \vspace{-2mm} % 控制上下间距
    % 右下 c 图
    % \ref{plotsub_b}\\
    \subfigure[Hallucination in different input contexts]{
    \setlength{\abovecaptionskip}{-25pt} % 调整标题与图片之间的间距
        \begin{tikzpicture}[scale=0.75]
            \begin{axis}[
                grid=major,
                ybar=0.2pt,
                bar width=0.45cm,
                enlarge x limits=0.17,
                width=1.2\textwidth,
                height=0.35\textwidth,
                % xlabel={\textbf{\huge Model}}, 
                xtick=data,
                xticklabels={CL-7B, CL-13B, DSC-1.3B, DSC-6.7B},
                ymin=0.45, ymax=1.19,
                legend style={at={(0.95,1.25)}, anchor=east,legend columns=-1,draw=none,font=\large},
                legend image code/.code={
            \draw [#1] (0cm,-0.08cm) rectangle (0.4cm,0.1cm); },
                legend image post style={scale=0.9, thick},
                % legend to name = plotsub_b,
                legend cell align={left}, % 图例文字左对齐
                tick align=outside,
                xticklabel style={font=\normalsize},
                yticklabel style={font=\large},
                % ticklabel style={font=\LARGE},
                every axis plot/.append style={line width=1pt},
                every axis/.append style={line width=1pt},
                ylabel={\textbf{\large MaHR}}, 
                nodes near coords,
                nodes near coords style={font=\large,xshift=3pt}
            ]
            \addplot[fill=p1, nodes near coords, every node near coord/.append style={yshift=5pt}] table[x=datasets, y=base]{\dskfive};
            \addplot[fill=p2, nodes near coords, every node near coord/.append style={yshift=4pt}] table[x=datasets, y=RAG]{\dskfive};
            \addplot[fill=p3, nodes near coords, every node near coord/.append style={yshift=-1pt,xshift=-1pt}] table[x=datasets, y=P-C]{\dskfive};
            \addplot[fill=p4] table[x=datasets, y=API-G]{\dskfive};
            \legend{{\normalem Base}, {\normalem RAG}, {\normalem Project files}, {\normalem API reference}};
            \end{axis}
        \end{tikzpicture}
        \label{fig:sub_c}
        \setlength{\belowcaptionskip}{-25pt} % 调整标题与图片之间的间距
    }
\end{minipage}
% \vspace{-2.5mm} % 控制上下间距
\caption{Analysis of API hallucinations across different dimensions.}
\label{fig:RQ4_CR}
\end{figure*}



\noindent \textbf{Contributions.} The main contributions of our paper are summarized below:

\begin{itemize}[leftmargin=*]
     \item To the best of our knowledge, we are the first to systematically investigate API hallucination in the code generation process under practical scenarios and propose one benchmark and two metrics.

    \item We propose {\tool}, a novel framework that supplements hierarchical dependencies externally and constrains the decoding process internally, %together
    mitigating API hallucination in the code generation process of LLMs.
    
    \item We evaluate {\tool} on both open-source and industrial scenarios. Experimental results show that our framework outperforms baselines, effectively and efficiently mitigating API hallucination and improving code generation quality.
    
\end{itemize}

% \noindent \textbf{Outlines.}



% However, LCMs still face notable challenges in industrial development scenarios, where models need to complete API calls within large, multi-file projects~\cite{}. In such contexts, models must handle repository-level information, such as project-specific APIs defined across various files or third-party library APIs. Failure to account for these global dependencies can result in ``API hallucination'', where models generate incorrect or non-existent API calls~\cite{}. As illustrated in Figure~\ref{}, [example description]. The consequences of API hallucinations are far-reaching, not only propagating errors throughout the codebase and increasing debugging complexity but also introducing potential security vulnerabilities. A recent study reports that 29\% of security vulnerabilities in the Linux kernel in 2021 were traced back to improper API usage~\cite{}. Given this severe impact, 
% exploring effective mitigation methods has become a critical research focus. Existing studies primarily adopt Retrieval-Augmented Generation (RAG) techniques to mitigate API hallucinations~\cite{}. These methods typically involve constructing a retrieval library containing API documentation or segmented repository code, retrieving relevant information based on the current function, and integrating this information to guide LCM's API completion process. While RAG-based solutions have shown some success, they face two major limitations. 

% \textit{1) Maintenance of retrieval libraries.} Maintaining up-to-date libraries is labor-intensive due to the rapid evolution of software libraries and frameworks (e.g., Java's most widely used libraries underwent over [X] API changes in the past [Y] years [citation]) and frequent changes in project repositories (e.g., popular open-source projects on GitHub undergo substantial code changes every 2-3 days on average [citation]). Outdated retrieval libraries can lead to incorrect or outdated API completion, potentially introducing bugs or compatibility issues in the developed software.

% \textit{2) Efficiency constraints for real-time deployment.} Developers expect AI-powered coding assistants to respond within xx milliseconds [citation] to maintain a seamless workflow. However, RAG-based methods often struggle to meet these time constraints due to retrieval and iterative processes, which can double or triple the overall latency. Excessive latency in API completion can greatly disrupt user experience, leading to reduced productivity and potential disengagement from the AI assistance tool. 

% These limitations highlight the need for a more efficient and context-aware approach to mitigating API hallucinations, which could capture and utilize project contextual information while maintaining low latency for real-time API completion.

% \noindent \textbf{Our work.} In this paper, we propose {\tool}, a novel framework designed to mitigate API hallucination in LLMs through multi-view context intervened decoding. Our key insight is to leverage rich project knowledge to supplement context dependencies externally and intervene in the generation process internally. 
% Specifically, {\tool} comprises two phases: \textit{1) {\phaseone}.} This phase captures multi-view dependencies based on the relevance between the current function and repository content. It aims to integrate an informative project skeleton into high-quality API completion prompts within the model's context window limits. \textit{2) {\phasetwo}.} This phase employs a token-level intervention mechanism, constraining the decoding space to valid API candidates through dynamic masking based on a prefix tree structure. It aims to enforce type consistency in API completions and reduce hallucinations. 

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/fig1API-type.pdf}
%     \caption{xxxx}
%     \label{fig:API-type}
% \end{figure}

% \textit{1) Ignoring project structural dependencies.} When developers call APIs, they typically consider dependencies of the current code snippet on other functions and modules, which guide the proper API usage within the project context. However, existing approaches ignore these important structural dependencies, providing only isolated code snippets as references for LLMs. As shown in Figure~\ref{}, [the des of current function]. Although the retrieved code demonstrates similar [xxx] functionality, it lacks essential structural context about the current function's dependencies, such as the imported class ``xxx'', leading to incorrect API generation.



==> FSE25-Industry-APIMitigation_2/sections/2_motivatingExample.tex <==



\section{PRELIMINARY STUDY} \label{sec:motivation}
To better understand API hallucination in the industrial scenario, we conduct a preliminary study using a Huawei internal project. The study explores the prevalence of hallucinations across different API types and input contexts. We collect a dataset of 200 code snippets, including 100 third-party library API calls and 100 project-specific API calls, covering common API usage patterns in industrial software~\cite{api-type}, as shown in Figure~\ref{fig:sub_a}. The evaluation involves four widely-used LLMs, including CodeLlama-7B/13B~\cite{codellama} and DeepSeek-Coder-1.3B/6.7B~\cite{deepseek}, and a metric for measuring the portion of hallucinated APIs, named MaHR.

\subsection{Hallucination in Different API Types}

We input the collected code snippets into the four LLMs and analyze the proportion of hallucinated APIs. As shown in Figure~\ref{fig:sub_b}, the models generate few hallucinations for third-party library APIs, with an average rate of only 12.75\%. However, for project-specific APIs, the hallucination rate is much higher, averaging 85.25\%. This indicates that while models handle third-party library APIs well due to their frequent presence in training data, they struggle with project-specific APIs due to a lack of contextual awareness. 
Notably, larger models show only marginal improvements in reducing hallucinations compared to smaller models, indicating that increasing model size alone is insufficient to address this issue. 
These findings highlight the challenge of API hallucination in industrial scenarios, especially for project-specific APIs.


\subsection{Impact of Different Input Contexts}

To further explore ways to mitigate hallucination in project-specific APIs, we design four input context scenarios: (1) \textit{Base}, only using the collected code snippets; (2) \textit{RAG}~\cite{zhang2024llm}, using BM-25 to retrieve similar code snippets from the project; (3) \textit{Project files}, including all project files randomly; (4) \textit{API reference}, explicitly providing validated APIs as guidance. The results are shown in Figure~\ref{fig:sub_c}, and we make the following observations:

\begin{itemize}

    \item \textbf{Observation 1:} Including more project information (Scenario 3) improves performance and even outperforms the RAG-based approach (Scenario 2). This highlights the importance of a broader project context for API hallucination mitigation. However, due to context window limits, it is not feasible to include all project files.

    \item \textbf{Observation 2:}Including API references in the input context (Scenario 4) helps reduce some hallucinations, but the rates remain still very high, averaging 44\% across four models. This indicates that API references alone are insufficient to fully guide the model toward accurate API generation.
    
\end{itemize}

In summary, our study highlights the challenges of mitigating API hallucination, particularly for project-specific APIs. While a broader project context improves performance, it is limited by input constraints. Additionally, providing API information alone fails to reduce the hallucination issue.
% ensure accurate usage. 
These results emphasize the need for more effective approaches
% strategies 
to address API hallucination in industrial development.


==> FSE25-Industry-APIMitigation_2/sections/2_preStudy.tex <==
% API hallucination, in which large language models (LLMs) incorrectly generate API-related code, has become a critical challenge in software engineering tasks. To evaluate and analyze this phenomenon, several benchmarks have been introduced. For example, the recently proposed CrossCodeEval~\cite{ding_crosscodeeval_2023} focuses primarily on cross-file code completion, but ignores the widespread reliance on third-party libraries in real-world software development. CloudAPIBench~\cite{jain_mitigating_2024} explores the use of third-party APIs. However, it does not incorporate project-specific APIs, lacking a comprehensive evaluation of project-level contextual dependencies.

% Given that both API type and API call frequency significantly influence model performance, we propose APIHulBench, a benchmark designed to evaluate API hallucination across varying frequencies (high-frequency and low-frequency APIs) and types (third-party and project-specific APIs). By conducting extensive evaluations on multiple state-of-the-art LLMs, our work provides an in-depth analysis of how different API characteristics impact hallucination. We reveal key sources of confusion that contribute to API hallucinations and provide targeted insights for subsequent research on mitigating API hallucinations.


\modify{While previous studies have identified the phenomenon of API hallucination in LLMs~\cite{}, there is still a lack of comprehensive studies exploring its characteristics and mitigation strategies. To fill this gap, we introduce {\dataset}, a comprehensive benchmark for evaluating real-world API hallucinations. We then evaluate four representative LLMs on {\dataset} to investigate hallucination patterns across various API types, offering valuable insights for developing effective mitigation strategies.}
 
\subsection{{\dataset}} \label{sec:benchmark}

% 

\subsubsection{Benchmark Construction }

\textit{Dataset Collection.}

\textit{API Type Annotations.}

\textit{API Frequency Annotations.}


\subsubsection{Format and Statistics}


\textit{Data Format.}


\textit{Data Statistics.} As a result, we obtain xxxx. 

In this section, we aim to 

briefly describe how we collect software repositories, select a subset of them for the {\dataset} construction, classify the APIs called from the selected repositories in terms of type and frequency, and APIHulBench statistics. The APIHulBench construction process is illustrated in ~\ref{fig:benchmark}. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/benchmark.png}
    \caption{The APIHulBench construction process.}
    \label{fig:benchmark}
\end{figure}

\textbf{Dataset Collection.} We 

collected over 99 stars of Java repositories from GitHub and then filtered out repositories with code files larger than 1,000, ending up with 10,605 repositories. These repositories will be used for third-party API call frequency statistics. In general, when building benchmarks for code LLMs, it is essential to reduce data leakage, i.e., we must ensure that the data in the benchmarks are not trained by the models. Therefore, we focus on recently created repositories. Specifically, we filtered out repositories created after 2023 from the 10,605 repositories collected, totaling 244 repositories. This ensures that the amount of data collected is large enough and does not overlap with the training data of many existing large code models released before 2023, avoiding underestimation of the API hallucination rate.


\textbf{API Type Annotations.} In order to distinguish the external knowledge required by different types of APIs, we classify API calls into two categories: project-specific APIs and third-party APIs. First,we parse each file in the repository and extract file-level imported libraries. The imported libraries are usually explicitly declared through import statements and reflect the classes and libraries the current file depends on. Next, based on the path information of the imported libraries, they match the file structure of the repository. If the path to an imported library can be found in the current project's directory, the imported library is considered an internal library, and it is inferred that the API call belongs to a project-specific API; otherwise, if the path to the imported library is not in the project's repository, but comes from an external dependency (e.g., the Java Standard Library, third-party libraries, or frameworks), the imported library is labeled as an external library, and the associated API call is classified as a third-party APIs.


\textbf{API Frequency Annotations.} In order to explore whether there is a difference in the hallucination rate of APIs with different frequencies in LLMs/LCMs, APIHubBench further categorises the frequency of API usage. Based on the classification of API types, we statistically analysed the frequency of third-party API calls using data collected from 10,605 code repositories. Due to the sufficiently large size of the data, these 10,605 code repositories can be considered as a reasonable approximation of the distribution of real-world APIs. Therefore, we can use them to explore the relationship between the hallucination rate of various code LLMs and the API frequency. Specifically, we filtered 244 target repositories from 10,605 code repositories and counted the frequency of third-party API calls in these repositories. Subsequently, based on the number of occurrences of APIs in the 10,605 repositories, we classify APIs into two categories: low-frequency APIs (\(\leq 10\) invocations) and high-frequency APIs (\(\geq 100\) invocations). This classification method follows the idea of grouping concepts by their popularity or frequency in pre-trained data~\cite{mallen_when_2023}~\cite{razeghi_impact_2022}.

\input{datas/benchmark-statistics}

\textbf{Construction.} Our purpose of constructing the APIHulBench was to extend the classification on the API hallucination. Thus we classified APIs into project- specificed kinds and third-party kinds, and among third-party APIs we further classified them into high-frequency and low-freqwuency APIs, which eventually yielded 1073 project- specificed APIs, 1603 third-party high-frequency APIs and 139 third-party low-frequency APIs, respectively. The statistics of APIHulBench are presented in table1(). For each api data, we add three levels of information, repo-level, file-level and function-level.Specific information on the three levels is as follows:
\begin{itemize}
\item {\textbf{Repo-level information}} includes the name of the repository, an overall description of the repository, and the external libraries or frameworks that the repository depends on.
\item {\textbf{File-level information}} includes import information in the file, class, function, and variable definitions defined in the file, and comments in the header or significant parts of the file.
\item {\textbf{Function-level information}} includes the name of the function, the name of the class to which it belongs, the signature of the function, the function's documentation string, the function's parameters and their types, the context of the function's code fragment, information about the target API called in the function, other internal methods called by the function, and external libraries called in the function.
\end{itemize}

\subsection{Studied Baselines} \label{sec:preStudy baseline}
\quad In order to initially evaluate the performance of the model on different types and frequencies of APIs, we extracted part of the data from APIHulBench, and the extraction process prioritized the diversity of the data to ensure that the data on the same category came from different repositories, and finally extracted 131 project-specified API data, 179 third-party high-frequency API data and 161 third-party low-frequency API data. As shown in Table(), we selected four representative LLMs (Llama-7B~\cite{}, Deepseek-33B~\cite{}, StarCoder2-15b~\cite{}, GPT-4~\cite{}) for evaluation. These four models cover a wide range of sizes and training objectives, from small to large models, and encompass state-of-the-art large code modelling techniques. 

\subsection{Metrics} \label{sec:metrics}
\quad In our preliminary study on exploring the performance of different types and frequencies of APIs in LLM, we mainly used \textbf{Exact Match (EM)}, \textbf{Editorial Similarity (ES)} and \textbf{Identifier Matching} as evaluation metrics. Taking into account elements such as identifiers, keywords, operators and delimiters, the EM and ES metrics help evaluate the overall accuracy of the code completion process. The identifier matching metric evaluates the ability of the model to generate the correct Application Programming Interface (API). For the evaluation, we parse the code and extracted identifiers from model generations, which are compared against the ground-truth identifiers to compute the F1 score.

Additionally, to quantify a Code LLM's uncertainty during API invocation, we define \textbf{API invocation confidence} as the minimum probability among all predicted API name tokens.~\cite{} Because the API name represents the core function or operation being invoked and has a large impact on subsequent reasoning, we focus only on the invocation confidence of the API name.

Furthermore, based on the correctness of the API calls, we classify the results into four types to more precisely analyze the sources of confusion in the model~\cite{}:

\textbf{Type 1: Completely Correct. }This type indicates that the model accurately generated both the correct API name and parameters, resulting in a fully correct API call.

\textbf{Type 2: API Name Correct.} Parameters Incorrect: This type indicates that the model successfully predicted the correct API name but made errors in the parameters. 

\textbf{Type 3: Incorrect but Existing API Called. }This type indicates that the model selected an incorrect API, even though the API exists in an external library or the project. 

\textbf{Type 4: Non-existent API Called.} THis type can be caused by two reasons,  either the API does not exist in the repository, or the API is not available in the external library that the model is calling. It reflects the model's lack of knowledge or misunderstanding of the external library.


\subsection{Results} \label{sec:result}

\quad Table 1() shows the performance of the model on different types and frequencies of APIs. Based on the experimental results, we derive the following findings:



Analysing this xx, we obxxx. 

\textbf{Observation 1.} [xxx]

\textbf{Observation 2.} [xxx]

Therefore, in this work, we propose to xxx.

\textbf{API type and frequency have a significant impact on the generation of model hallucinations.} Regarding API frequency, we observe a strong correlation between API frequency and effective API calls. On the other hand, in terms of API type, project-specific APIs are much more likely to hallucinate than high-frequency third-party APIs, but only slightly more likely than low-frequency third-party APIs. This suggests that the model lacks sufficient training data for low-frequency APIs, and lacks sufficient contextual knowledge for project-specific APIs, both of which tend to have higher hallucination rates.

\textbf{There is a strong correlation between API call accuracy and API call confidence.} Experiments have shown that the accuracy rate of API calls tends to be positively correlated with the API call confidence when the model predicts API names. When the model has higher API call prediction confidence, call accuracy is correspondingly higher. This finding indicates that API Invocation Confidence can be an important indicator of a model's prediction reliability.

\textbf{There are differences in the knowledge required for different types of APIs.} For third-party APIs, the main source of confusion for the model comes from ``calling the wrong but existing API'' (Type 3). This type of error is usually due to the model choosing a semantically or syntactically valid API in an external library or framework that is not applicable in the current context, reflecting the model's limited understanding of the external knowledge. For project-specific APIs, the model's main confusion stems from “calling an API that does not exist” (Type 4). This type of error may be due to the lack of accurate modeling of the project context in the model for project-specific APIs, resulting in the generated API names not matching the actual project. This further suggests that the model requires richer project-level contextual information and customization knowledge when dealing with project-specific APIs. This difference further reveals the different emphasis of the two types of APIs on relying on knowledge and contextual information external to the model.


==> FSE25-Industry-APIMitigation_2/sections/3_approach.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.52]{figures/framework.pdf}
    \caption{The overview of {\tool}.}
    \label{fig:framework}
\end{figure*}


In this section, we propose {\tool}, a framework to mitigate API hallucination in code generated by LLMs with hierarchical dependency aware. We first present the overview of {\tool} and then describe its details in the following subsections.

\subsection{Overview}

Given a project and an incomplete function, {\tool} generates a complete API call by a two-phase approach: (1) In the \textit{hierarchical dependency mining} phase, it extracts both local dependencies (i.e., called functions and reference APIs) and global dependencies (i.e., related files and the current file), enriching the input prompt to provide better context for LLM. (2) In the \textit{dependency constrained decoding} phase, the extracted dependencies are used to guide the generated API calls to align with the project's specifications by constructing valid API name prefix trees and identifying parameter patterns.
% During decoding, the constraints are applied to mask invalid logits, ensuring that the generated API calls align with the project's specifications.}

% \textcolor{blue}{(1) it performs hierarchical dependency mining by extracting both local dependencies (i.e., called functions and reference APIs) and global dependencies (i.e., related files and the current file). Incorporating these dependencies into the input prompt, it enriches the project context provided to the LLM; 
% (2) it applies dependency constrained decoding by preprocessing the extracted dependencies to construct an API name prefix tree and valid parameter patterns, dynamically applying these constraints during decoding by masking invalid logits to ensure generated tokens adhere to the project's API specifications. }


\subsection{{\phaseone}}

As shown in Figure~\ref{fig:framework} {\large\ding{182}}, {\tool} analyzes dependencies at two levels: local (function-level) and global (file-level), constructing a hierarchical structure of the project. This structure decomposes the project top-down, from files down to detailed functions. Beyond explicit structural relationships, it also incorporates implicit reference dependencies (See Section~\ref{sec:global}). Therefore, it provides a rich context for code generation that spans both immediate function details and broader project architecture.

\subsubsection{Local Dependency Analysis}

It focuses on the immediate context of the incomplete function. Through static analysis, we first identify valid APIs available at the generation position, providing clear references for the LLM's output. We also analyze method dependencies, including functions called within the same file or across other files in the project. This process captures both function calls and data flow, offering detailed relationships surrounding the incomplete function.

\subsubsection{Global Dependency Analysis} \label{sec:global}

While local dependencies provide immediate context, understanding broader project relationships is crucial for generating code within a large project, which is the global dependency. For the unfinished function, we first leverage static analysis to extract the import statements in its current file and then identify all imported files. These related files provide essential context about the available methods for the current function. To avoid overwhelming LLMs and exceeding input length limits, we extract a concise ``skeleton'' of these files. Specifically, for each file, we preserve its class definitions, field declarations, and function signatures while excluding detailed implementations. This approach provides a compact yet informative representation of the global dependency on projects.

% While local dependencies provide immediate context, generating code in large projects requires understanding broader file relationships. 

% we focus on the current file To address this, we use static analysis to extract the import statements from the current file, identifying the related files, which xxxx. To avoid overwhelming the LLM and exceeding its input length, we simplify the file's information into a ``skeleton''. For related files, we retain class definitions to outline high-level components, as well as member fields and method signatures to represent their functionality \cuiyun{[???]}. 
% \modify{For the current file}, we focus on three key elements: its import statements, defined fields, and defined functions.
% This streamlined representation ensures the LLM receives the necessary context without unnecessary details, enabling efficient code generation.

% 1) for files, we keep class definitions to show high-level components; 2) for classes, we include member fields and methods to capture functionality; 3) for methods, we retain signatures to clarify input and output. For present files, we extract 1) import statements 2) defined fields 3) defined Functions. 

\begin{figure}
    \centering
    \setlength{\belowcaptionskip}{-3pt} % 调整标题与图片之间的间距
    \includegraphics[scale=0.47]{figures/approach_prompt.pdf}
    \caption{An example illustrating the {\tool}' prompt template based on the incomplete function in Section~\ref{sec:intro}.}
    \label{fig:prompt}
\end{figure}
\subsubsection{Input Prompt Construction}

Based on the dependency analysis, we construct a structured input prompt, as illustrated in Figure~\ref{fig:prompt}. This prompt integrates the following key components:

\begin{itemize}[leftmargin=*]
    \item \textbf{Project Description.} A brief overview of the project's purpose, providing essential background for the LLM.

    \item \textbf{Global Dependency.} Simplified skeletons of related and current
    % present 
    files, including class definitions, member fields, and function signatures, to represent the broader project structure.

    \item \textbf{Local Dependency.} Called functions and reference APIs that are directly relevant to the incomplete function, serving as %capturing 
    its immediate context.
    
    \item \textbf{Incomplete Function.} The partially implemented target function, with the {\tt[API\_Position]} marking the location where the API call should be generated.
    
\end{itemize}

\subsection{{\phasetwo}}

This phase first analyzes the mined dependencies to preprocess valid API-related information and then integrates these constraints into the decoding process, as illustrated in Figure~\ref{fig:framework}{\large\ding{183}}. 

\subsubsection{Dependency Preprocessing} In this step, dependencies are used to build an API name prefix tree and identify parameter patterns, forming a constrained set of valid options. These valid tokens are cached to ensure efficient access during decoding, as shown in Figure~\ref{fig:framework}{\large\ding{183}-I}. 

% For APIs, we preprocess both name and parameter to establish a constraint \fgd{tree, } %xxxx , 
% as shown in the top part of Figure~\ref{fig:framework}\ding{2}.

\textbf{API name prefix tree.} Given a reference API set $\mathcal{A}=\{a_1, a_2, \cdots a_n\}$, %we map each API $a_i$ to its token representation $\mathcal{T}(a_i)$ in the LLM's vocabulary space $V$. 
we tokenize the name of each API $a_i$ to $\mathcal{T}(a_i)$ based on the LLM's vocabulary. It is
% It’s 
important to note that tokenization in LLMs is context-dependent. For example, in CodeLlama-7B, the tokenization sequence for {\tt willReact} is [674, 1123, 627], but in the context of {\tt reaction.willReact}, it becomes [14043, 1123, 627]. To ensure consistent tokenization, we tokenize both the full API calls and their prefixes (i.e., the tokens before the last ``.''). We then remove the shared prefixes, yielding a deterministic representation $\mathcal{T}(a_i)$ for each API. In real-world projects, reference APIs often share common prefixes. For efficient constraint validation during generation, we construct a prefix tree from these APIs' token sequences, as described in Algorithm~\ref{alg:trie}. The algorithm initializes the tree with an empty root node (line 1) and iterates through each reference API (line 2). For each token in the tokenized API, it builds the tree recursively (lines 3-8): if a token is not a child of the current node, a new node is created (lines 4-5), then the algorithm moves to this child node (line 7). Upon completion, each root-to-leaf path in the tree represents a complete API token sequence, enabling efficient validation of generated API calls.

% , where each node $v \in V$ represents a token, each $(v_i,v_j) \in E$ indicates valid token transitions and each root-to-leaf path represents a complete API token sequence. The construction process is detailed in Algorithm~\ref{alg:trie}.

\begin{algorithm}[t]
  \caption{Prefix Tree Construction for API Tokens}
  \label{alg:trie}
  \small
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \Input{Reference APIs $\mathcal{A}$, Tokenizer $\mathcal{T}$}
  \Output{Prefix tree $G$}
  % \BlankLine
    Initialize the prefix tree $G$ with a root node $\mathcal{R}$, where $\mathcal{R}$.child $\gets \emptyset$\;
  \ForEach{ $a_i \in \mathcal{A}$}{
  \tcp{\textcolor{teal}{recursively build the prefix tree;}}
      \ForEach{$t_i \in \mathcal{T}(a_i)$}{
          \If{$t_i \notin \mathcal{R}$.child}{
              \tcp{\textcolor{teal}{add $t_i$ into the children of $\mathcal{R}$;}}
              $\mathcal{R}.$child[$t_i$] $\gets$ create a new node with $t_i$\;
          }
        $\mathcal{R}\gets \mathcal{R}$.child[$t_i$]\;
        
      }
  }
  \Return{$\mathcal{R}$}\;

  % \BlankLine
  % \SetKwFunction{CreateNode}{\tt CreateNode}
  % \SetKwProg{Fn}{Function}{:}{}
  % \Fn{\CreateNode{$\mathcal{R}$, $t_i$}}{
  %     $c \gets$ create a new node based on $t_i$\;
  %     $\mathcal{R}$.child[$t_i$] $\gets c_i$\;
  % }
\end{algorithm}


% A minimalistic trie node can be defined as an one-to-one dict mapping token_ids (keys) to its child nodes(values).  Any trie operations thus can be peformed by traversing from the root node to its children.

% To build the token trie of a specific entity, we began by inserting one api tokens sequence to the trie. As demonstrated in the `INSERTION` function, we simply creating new child nodes (if not exist) and pointing current nodes to them until running out of tokens. The trie construction shall be completed when we finish inserting every token sequence. 

% [Construction details?
% Specifically, for all tokenized APIs $\{T(a_1),T(a_2),...,T(a_n)\}$, we:
% 1. Initialize an empty trie with a root node $r$
% 2. For For each token sequence $T(a_i) = [t_1, t_2, ... ,t_n]$:
% Start from root node $r$
% For each token $t_j$ in sequence:
% If current node has no child with token $t_j$, create new node
% Add edge to child node with token $t_j$
% Move to child node
% Mark final node as leaf]

\textbf{Parameter Patterns.} We use an indicator function $I$ to differentiate between APIs with and without parameters. To handle parameter-related tokens in the LLM vocabulary, we classify them into two categories:

\begin{itemize}[leftmargin=*]
    \item $B_{noparam}$: Tokens representing no-parameter patterns (e.g., ``())'', ``()))\{'') that appear when an API is called without arguments.

     \item $B_{param}$: Tokens representing parameter patterns (e.g., ``([\text{--}'', ``(@'') that indicate the start of parameter lists.
\end{itemize}

\subsubsection{Constrained Decoding} As shown in Figure~\ref{fig:framework}{\large\ding{183}-II}, at each step $t$, the LLM outputs logits $l \in \mathbb{R}^{|V|} $ representing token probabilities over its vocabulary $V$. To ensure the generated APIs conform to mined dependencies, we employ an adaptive 
% a dynamic 
masking mechanism that combines both API name and parameter pattern constraints. 

Given the current sequence $\{t_1, t_2, ..., t_k\}$, if $t_{k+1}$ is an API name token, we locate the current node in the trie structure and collect valid next tokens from its children as $V_{valid} = \{ v| v \in n.children\}$. if $t_{k+1}$ is a parameter token,  we consult the parameter indicator $I$ to determine valid tokens - allowing only no-parameter tokens when $I=0$ or parameter tokens when $I=1$.
% For the API name, we first locate the current node in trie $G$ and collect valid next tokens from all child nodes $V_{valid} = \{ v| v \in n.children\}$. 
% utilize the preprocessed trie structure $G$ to validate token sequences. Specifically, 
% given the current generated token sequence $\{t_1, t_2, ..., t_k\}$, we locate the current node in trie $G$ and collect valid next tokens from all child nodes $V_{valid} = \{ v| v \in n.children\}$.
% % \textbf{Parameter Pattern Decoding.} 
% 
% it is controlled by indicator $I$. Based on the API's parameter requirements, we allow only no-parameter tokens ($B_{noparam}$) when $I=0$ and parameter-starting tokens ($B_{param}$) when $I=1$. 
These constraints are integrated into a unified binary mask $M \in \{  0,1\}^{|V|}$:

\begin{equation}
M_i = \begin{cases}
1 & \text{if } i \in V_{valid} \text{ (API name constraint)} \\
1 & \text{if } i \in B_{noparam} \text{ and } I = 0 \text{ (no-param constraint)} \\
1 & \text{if } i \in B_{param} \text{ and } I = 1 \text{ (param constraint)} \\
0 & \text{otherwise}
\end{cases}
\end{equation}

The constrained logits are then computed through element-wise multiplication $l_{masked} = l \odot M$, and the next token is selected via greedy search: 
\begin{equation}
 t_{(k+1)}=argmax_t(softmax(l_{masked})).
\end{equation}
This process iterates until a complete API call is generated or a maximum length is reached.

% % We then construct a binary mask $M \in \{  0,1\}^{|V|}$, where $ M_i = 1$  if token $i$ in valid set $V_{valid}$, and 0 otherwise, effectively limiting the model's choices to only valid API tokens.

% % We constrain this distribution through a dynamic masking mechanism:
% % \begin{equation}
% % l_{masked} = l \odot M
% % \end{equation}

% During generation, we design a token-by-token constrained decoding process using dependency trie and parameter patterns.

% \textbf{Trie-based Token Constraint.}  Given an input prompt, the LLM generates tokens sequentially. At each generation step $t$, the model produces a probability distribution over its vocabulary $V$ in the form of logits $l \in \mathbb{R}^{|V|} $. To constrain this distribution, we first locate current position in the dependency trie based on the generated token sequence $t_1, t_2, ..., t_k$. From this position, we identify all valid next tokens $V_{valid}$ by collecting the tokens from all child nodes. We then construct a binary mask $M \in \{  0,1\}^{|V|}$, where $ M_i = 1$  if token $i$ in valid set $V_{valid}$, and 0 otherwise, effectively limiting the model's choices to only valid API tokens.

% \textbf{Parameter Pattern Handling.} 
% % 

% For parameter pattern generation, we maintain two token sets: $B_{nopara}$ in which tokens representing parameter-free patterns (e.g., ``()'') and $B_{param}$ in which tokens representing parameterized patterns (e.g., ``('', ``)''). When generating parameter tokens, we extend the mask $M$ based on the API's parameter flag $f$:

% \begin{equation}
% M_i =
% \begin{cases}
% 1, & \text{if } i \in B_{noparam} \text{ and } f = 0, \\
% 1, & \text{if } i \in B_{param} \text{ and } f = 1, \\
% M_i, & \text{otherwise}.
% \end{cases}
% \end{equation}

% Finally, we apply the mask to the original logits:
% \begin{equation}
% l_{masked} = l \odot M
% \end{equation}
% where $\odot$ denotes element-wise multiplication.

% This masked distribution ensures that only validated API tokens can be selected while maintaining correct parameter patterns and coherence with project dependencies.

% \begin{algorithm}[h]
%   \caption{The Construction of Prefix Tree}
%   \label{alg:framework}
%   \small
%    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%     \Input{}
%     \Output{}
%     $f \gets$ {\tt False}; $\underline{\rho} \gets k^* / 2$; $\overline{\rho} \gets k^*$; $\mathbf{w} \gets \emptyset$ \; 
%     \Repeat{$f$={\tt True}}{
%         \tcp{\textcolor{teal}{(1) The graph reduction method.}}
%         $G\gets${\tt  ReduceGraph}($G$, $\underline{\rho}$)\;
        
%         \tcp{\textcolor{teal}{(2) The vertex weight update method.}}
%         $\mathbf{w} \gets$ {\tt VWU}($G$, $\mathbf{w}$, $T$, $\underline{\rho}$, $\overline{\rho}$)\;
        
%         \tcp{\textcolor{teal}{(3) The candidate subgraph extract and verify.}}
%         $(f, \mathcal{D}(G), \underline{\rho}, \overline{\rho}) \gets$ {\tt CSV}($G,\underline{\rho}, \overline{\rho}, \mathbf{w}$, $\epsilon$);
        
%         % \tcp{\textcolor{teal}{(4) The result verify method.}}
%         % $(f, \mathcal{D}(G)) \gets$ {\tt Verify}($S,\mathbf{w}$, $\underline{\rho}$, $\overline{\rho} $, $\epsilon$)\;
    
%     }
    
%     \Return{$\mathcal{D}(G)$;}

% \end{algorithm}

==> FSE25-Industry-APIMitigation_2/sections/4_setup.tex <==

\subsection{Research Questions} \label{sec:RQ}

In this paper, we mainly investigate the following research questions through experiments.

\begin{itemize}[leftmargin=*]

\item {\textbf{RQ1:}} How effective is {\tool} in mitigating API hallucination on {\dataset}?
\item {\textbf{RQ2:}} What are the impacts of two components in {\tool} (i.e., \textit{hierarchical dependency mining} and \textit{dependency constrained decoding})?
\item {\textbf{RQ3:}} How efficient is {\tool} compared to baseline approaches?
\item {\textbf{RQ4:}} How does {\tool} perform in mitigating API hallucination in an industrial scenario?
\end{itemize}

\subsection{Benchmarks} \label{sec:benchmark}

% Since existing API hallucination evaluation benchmarks suffer from potential data leakage from older project~\cite{} and reliance on model-synthesized data~\cite{}, we construct a new benchmark, named {\dataset}, whose key feature is the project-specific API calls in each sample, challenging models in practical development scenarios.

Existing API hallucination evaluation benchmarks face challenges such as potential data leakage from older projects~\cite{eghbali2024hallucinator} and reliance on model-synthesized data~\cite{tian2024codehalu,jain2024mitigating}. To address these issues, we construct a new benchmark, {\dataset}, which focuses on project-specific API calls in real development scenarios, providing a more practical evaluation of LLMs.

\subsubsection{Project Collection}
We collect Java projects from GitHub created between mid-2023 and mid-2024, ensuring they postdate the training cut-off dates of many existing code LLMs~\cite{benchmark-time}. To ensure quality, following prior work~\cite{bench_year}, we excluded projects with fewer than 10 files or fewer than 200 stars, resulting in a final dataset of 98 high-quality projects.

\subsubsection{Dataset Generation}
For each project, we use tree-sitter~\cite{tree-sitter} to parse Java files and extract functions with more than five lines as candidate samples. We identify project-specific API calls within these functions and split each function into two parts: the prompt (code before the API) and an inference part (containing the ground truth API). The line position of each API call is recorded. Following prior studies~\cite{benchmark-time,bench_year}, we eliminate duplicate prompts, resulting in a benchmark with 416 unique samples. 
To reflect different development stages, we divide the benchmark into two variants based on API call positions: 1) {\dataset}-F, including 221 samples where API calls appear in the first 50\% of the function lines, reflecting scenarios where developers are initiating their implementation and seeking early assistance. 2) {\dataset}-M, including 195 samples where API calls appear beyond the 50\% mark, simulating scenarios where developers have written most of the code and need assistance during later stages of development.
% 1) {\dataset}-F including 221 samples where API calls appear in the first 50\% of the function lines, simulating scenarios where developers seek early assistance.
% {\dataset}-M including samples 194 where API calls appear beyond the 50\% lines of the function lines, simulating scenarios where developers need assistance later in the development process. 
This division enables a more nuanced evaluation of LLM performance across different stages of coding, providing insights into their practical performance in real-world development.

\subsection{Studied LLMs} 

Following prior studies~\cite{wavecoder,Magicoder,zhang2024llm}, we adopt two widely-used LLMs for code generation with different model sizes:
% conduct a comprehensive comparison, we adopt two widely-used LLMs for code generation, considering different model sizes:

\begin{itemize}[leftmargin=*]
    \item \textbf{CodeLlama~\cite{codellama}} released by Meta AI, is further trained on Llama 2~\cite{llama2} with 0.5 trillion code-specific tokens. Our experiments use its 7B, 13B, and 34B versions.
    \item \textbf{DeepSeekCoder~\cite{deepseek}} released by DeepSeek AI, is a series of code-specialist LLMs trained on 2 Trillion tokens across over 80 programming languages. It achieves state-of-the-art performance among open-source code LLMs. Our experiments use its 1.3B, 6.7B, and 33B versions.
\end{itemize}


\subsection{Studied Baselines} \label{sec:baseline}

To evaluate the effectiveness of {\tool}, we compare it with the following baselines. Note that we do not include DAG~\cite{jain2024mitigating} in the comparison because this approach requires detailed documentation for each API, which is unavailable for many projects.

\begin{itemize}[leftmargin=*]

\item \textbf{Base Generation} is a default generation strategy using the current function as the input prompt.

\item \textbf{RAG~\cite{zhang2024llm}} retrieves code snippets from the project similar to the incomplete function and includes them in the input prompt.

\item \textbf{De-Hallucinator~\cite{eghbali2024hallucinator}} first generates code using the incomplete function. Then, it retrieves APIs related to this initial output, adds them to the input prompt, and iteratively refines the generation.

\end{itemize}

\subsection{Metrics}

To comprehensively evaluate the performance of LLMs, we focus on two aspects: generation accuracy and generation hallucination.

\subsubsection{Accuracy}

Following prior work~\cite{eghbali2024hallucinator}, we adopt three metrics to evaluate generation accuracy:

\begin{itemize}[leftmargin=*]

\item \textbf{Exact Match (EM)} measures the percentage of output that exactly matches the ground truth.

\item \textbf{Edit Similarity (ES)} calculates the Levenshtein distance between the output and the ground truth, normalized to a similarity score.

\item \textbf{Identifier Match (IM)} measures the percentage of output with correct API identifiers compared to the ground truth.

\end{itemize}

\subsubsection{Hallucination}

% In API-specific scenarios, 
We focus on two key elements in APIs, including the 
% API 
names and
% API 
parameter patterns, and
% Based on these elements, we 
introduce two new metrics for evaluating the degree of API hallucination.
% to evaluate API hallucination.

% Since the parameter types of generated API are difficult to analyze accurately, we focus on the number of parameters.
% Based on these facts, we introduce two new metrics from different levels to evaluate API hallucination.

\begin{itemize}[leftmargin=*]

\item \textbf{Micro Hallucination Number (MiHN)} counts the average number of hallucinatory elements within the generated APIs:

\begin{equation}
\text{MiHN} = \frac{\sum_{i=1}^{n} \text{Count}(hallucinatory \ elements \ in \ a_i)} {n},
\end{equation}
where $n$ is the total number of generated APIs, and $a_i$ is the $i$-th generated API.

\item \textbf{Macro Hallucination Rate (MaHR)} calculates the proportion of generated APIs that contain any hallucinatory elements:

\begin{equation}
\text{MaHR} = \frac{\text{Count}(APIs \ with \ hallucinations)} {n},
\end{equation}
where $n$ is the total number of generated APIs.

\end{itemize}

\subsection{Implementation Details}

Given the limited input size of 8,000 tokens, we restrict the project content to 7,000 tokens and the function content to 1,000 tokens (as the average length of incompetent function in our benchmark is 358). Content exceeding these limits is truncated from left to right, which ensures adequately and equally sized input windows for different baselines. The prompts of RAG~\cite{zhang2024llm} and De-Hallucinator~\cite{eghbali2024hallucinator} are constructed following their original papers. For a fair comparison, we run De-Hallucinator one iteration. We download all LLMs from HuggingFace Hub~\cite{HuggingFace}, use vllms~\cite{vllms} on Ascend as the inference and serving engine, and set the max\_new\_tokens parameter to 15. All experiments are conducted on a server with 192-kunpeng-920 CPU cores, 1.5T memory, hosted by EulerOS 2.1 Linux distribution, and equipped with 4 Ascend 910B-B3 64G NPUs. 

% [inference]
% 类似于有这些，但也不全是：【模型从哪里获取】，【并发】，【参数等】% [We acquire all models directly from their official open-source repositories. We employ the default greedydecoding strategy without sampling, since previous work [5] has illustrated the marginal differences between them in similar repositorylevel line completion scenarios. In the post-processing phase, we use beam search to generate the top-3 predictions as candidates, balancing accuracy with limited computational resources. Additionally, we define the termination condition for the generation process as the output of the first newline token to measure the accurate time cost of completing the whole line. We set the max_new_tokens parameter to 64 for all models. All experiments are conducted on a server with the Ubuntu 20.04.6 LTS operating system and equipped with eight A800-80G GPUs.]

 




==> FSE25-Industry-APIMitigation_2/sections/5_result.tex <==

\input{datas/RQ1_table}


\subsection{Effectiveness of {\tool} on {\dataset} (RQ1)}

\noindent \textbf{Experimental Design.} To answer this research question, we conduct experiments on the two benchmarks {\dataset}-F and {\dataset}-M using six different LLMs.

\noindent \textbf{Results.} Table~\ref{Table:res_main} shows that {\tool} consistently outperforms baseline approaches across all evaluated LLMs. 
% On average, MARIN improves the EM by 196\% and reduces MaHR by 406\%(times) compared to base models. 
Using the Wilcoxon signed-rank test~\cite{wilcoxon1992individual} (p-value < 0.001), we confirm the improvements are statistically significant.

\textbf{{\tool} can be tailored to various programming scenarios.} 
% {\dataset}-F represents early-stage programming with limited code context, while {\dataset}-M represents later-stage programming with more abundant context. 
The available content of incomplete function affects the base models' performance. For example, the six models achieve an average ES of 54.81\% and MaHR of 66.74\% on {\dataset}-M, while on {\dataset}-F, these metrics are 52.86\% and 69.67\%, respectively. {\tool} demonstrates strong performance in mitigating API hallucination across both scenarios. On {\dataset}-F, {\tool} improves the performance of the CodeLlama family by up to 175.39\% in EM while reducing MaHR by up to 80.15\% compared to RAG. On {\dataset}-M, similar gains are observed, with increasing up to 83.98\% in EM and reducing up to 79.62\% in MaHR. 
These results show {\tool} is well-suited for early-stage development with sparse context to later-stage tasks with richer dependencies.

\textbf{{\tool} shows generalization capability across various LLMs.} For DeepSeekCoder-1.3B, {\tool} boosts IM by 81.56\%, while reducing MiHN by 69.84\% compared to De-Hallucinator on {\dataset}-F. For larger models, DeepSeekCoder-33B, the impact remains substantial, improving IM by 87.06\% and reducing MiHN by 77.19\%. Similar trends are observed in the CodeLlama family. This generalization capability ensures {\tool} can be widely applied across different model architectures and sizes in diverse development scenarios.

\begin{tcolorbox}[breakable,width=\linewidth-2pt,boxrule=0pt,top=2pt, bottom=2pt, left=4pt,right=4pt, colback=gray!15,colframe=gray!15]
\textbf{Answer to RQ1:} {\tool} significantly mitigates API hallucination across diverse development scenarios and model sizes, achieving an average increase of 107.32\% in EM and an average decrease of 67.31\% in MaHR compared to the RAG approach.
\end{tcolorbox}


\input{datas/RQ2_figure}
\input{datas/RQ3_table}

\subsection{Impacts of Different Components in {\tool} (RQ2)}

\noindent \textbf{Experimental Design.} For this RQ, we perform ablation studies by considering different levels of dependencies with and without constrained decoding (CD), resulting in eight variants.

\begin{itemize}[leftmargin=*] 
\item \textbf{ALL w/wo CD:} Provides complete hierarchical dependencies, including both local and global dependencies. 
\item \textbf{-LD w/wo CD:} Removes local dependencies, providing only related files and the current file. 
\item \textbf{-GD w/wo CD:} Removes global dependencies, providing only called functions and reference APIs. 
\item \textbf{-LG w/wo CD:} Removes both local and global dependencies, providing only the incomplete function. \end{itemize}

\noindent \textbf{Results.} Figures~\ref{fig:res_aba_F} and \ref{fig:res_aba_m} show the performance of eight variants on {\dataset}-F and {\dataset}-M, respectively. The results confirm that both hierarchical dependencies and constrained decoding independently improve the performance of {\tool}, with their combination achieving the best results.

\textbf{Global dependency is more beneficial for hallucination mitigation.} Removing global dependencies (-GD) causes a larger performance drop. For example, on {\dataset}-F, removing global dependencies causes a 33.39\% drop in average EM and a 186\% rise in average MaHR across six LLMs. In contrast, removing local dependencies results in a 15.79\% decrease in average EM and an 81.66\% increase in average MaHR.
% , while similar trends are observed on {\dataset}-M, with EM dropping by 20.09\% and MaHR increasing by 27.52\%. 
This demonstrates that global dependencies, such as file structures and method signatures, are crucial for providing the context required for accurate API generation.
% Besides, removing both dependencies (-LG) causes the most severe performance degradation. On average, EM decreases by 58.46\% and MaHR increases by 167.2\% across both benchmarks. This highlights that the combination of local and global dependencies provides comprehensive structural information, which is crucial for effective hallucination mitigation. 
% Besides, removing local dependencies (-LD) results in a smaller performance decrease. On {\dataset}-F, the average EM decreases by 10.78\% and MaHR rises by 8.3\%, while on {\dataset}-M, EM drops by 8.89\% and MaHR rises by 7.09\%. This smaller impact suggests that function-level dependencies, while useful, are less critical than file-level dependencies in mitigating API hallucinations. Finally, 
% removing both dependencies (-LG) causes the most severe performance degradation. On average, EM decreases by 36.31\% and MaHR increases by 43.04\% across both benchmarks. This highlights that the combination of local and global dependencies provides comprehensive structural information, which is crucial for effective hallucination mitigation. 

\textbf{Constrained decoding consistently improves hallucination mitigation across different input contexts.} For complete dependencies (ALL), with constrained decoding, on {\dataset}-F, the average EM increases by 9.12 points and MaHR decreases by 11.53 points across six LLMs. On {\dataset}-M, the EM increases by 11.28 points and MaHR decreases by 12.22 points. Even in limited dependency settings (-LD, -GD, -LG), constrained decoding also achieves the improvements. For example, in ``-LG'' variant, constrained decoding improves the EM by an average of 8.52 points and reduces MaHR by an average of 16.13 points on {\dataset}-F across six LLMs.
These results highlight the effectiveness of constrained decoding could employ the available dependencies to prevent invalid API tokens in the generation process.
% \vspace{-2mm}
\begin{tcolorbox}[breakable,width=\linewidth-2pt,boxrule=0pt,top=1pt, bottom=1pt, left=4pt,right=4pt, colback=gray!15,colframe=gray!15]
\textbf{Answer to RQ2:} Both components are essential for the performance of {\tool}. Removing hierarchical dependency and constrained decoding leads to a performance decrease. Among these, global dependency is the most important module, having the greatest impact on overall performance.
\end{tcolorbox}
% \vspace{-2mm}
\subsection{Efficiency of {\tool} (RQ3)} 

\noindent \textbf{Experimental Design.} To evaluate the efficiency, we measure the computational time for all approaches. Due to computational resource constraints, we use 20 concurrent processes for LLMs with up to 10B parameters and 10 concurrent processes for LLMs with over 30B parameters. For each approach, we specifically measure:

\begin{itemize}[leftmargin=*] 
\item \textbf{Base:} The time required for model inference with only incomplete function. 
\item \textbf{RAG:} The total time for retrieval and model inference. 
\item \textbf{De-Hallucination:} The total time for initial inference, retrieval, and a secondary inference. 
\item \textbf{{\tool}:} The total time for static analysis and model inference, reflecting its dependency analysis and decoding phases. \end{itemize}
To ensure reliable results, the reported computational time for each approach is averaged across all test samples. 

\noindent \textbf{Results.} As shown in Table~\ref{table:res_efficiency}, {\tool} achieves comparable efficiency to base models while greatly outperforming RAG and De-Hallucinator in computational time across all model sizes and benchmarks. 
% On average, {\tool} adds only 0.001-0.073s of overhead compared to base models, whereas RAG and De-Hal. require 0.323-0.726s and 0.337-0.57s, respectively, demonstrating its lightweight design.

\textbf{{\tool} maintains consistent efficiency across various benchmarks.} Different development scenarios greatly impact the inference time of the base model, as six LLMs achieve fast inference with an average time of 0.203s on {\dataset}-F and 0.256s on {\dataset}-M, respectively. RAG experiences a substantial increase in time, adding 0.457s on {\dataset}-F and 0.706s on {\dataset}-M due to the retrieval process. De-Hallucinator, which requires iterative generation, introduces additional delays, with an overhead of 0.474s on {\dataset}-F and 0.482s on {\dataset}-M. In contrast, {\tool} adds only 0.024s on {\dataset}-F and 0.02s on {\dataset}-M, maintaining minimal computational overhead. 
% These results demonstrate that {\tool} is highly efficient across different development scenarios, maintaining minimal computational overhead while still achieving significant improvements in reducing hallucination.
This benefit stems from the {\tool}'s lightweight design (i,e., not rely on the expensive retrieval or iterative processes.).

\textbf{{\tool} exhibits superior scalability with increasing model size.} For example, in the DeepSeekCoder family, the smallest model (DSC-1.3B) completes inference in an average of 0.211s across two benchmarks. {\tool} adds only 0.007s overhead, while RAG and De-Hallucinator add 0.576s and 0.333s, respectively. For the largest model (DSC-33B), despite the base inference time increasing to 0.314s, {\tool} maintains a low additional overhead of 0.017s. In comparison, RAG adds 0.652s, and De-Hallucinator adds 0.547s. These results demonstrate that {\tool} exhibits superior scalability, maintaining minimal overhead regardless of model size.
% \vspace{-2mm}
\begin{tcolorbox}[breakable,width=\linewidth-2pt,boxrule=0pt,top=2pt, bottom=2pt, left=4pt,right=4pt, colback=gray!15,colframe=gray!15]
\textbf{Answer to RQ3:} {\tool} achieves comparable efficiency to base models, adding only 0.022s overhead on average. {\tool}'s lightweight design and superior scalability make it an efficient framework for mitigating API hallucination across diverse development scenarios and model sizes.
\end{tcolorbox}
% \vspace{-2mm}

\subsection{Performance of {\tool} in Industrial Scenario (RQ4)}

\input{datas/RQ4_table}

\noindent \textbf{Experimental Design.} To evaluate {\tool} in an industrial scenario, we construct a benchmark with 109 samples from Huawei's internal Java projects, following the process described in Section~\ref{sec:benchmark}. We use Huawei proprietary LLMs, PanguCoder-11B and PanguCoder-34B, as the base models for the experiments.

\noindent \textbf{Results.} The results in Table~\ref{table:res_industry} show that {\tool} outperforms baseline approaches in industrial scenarios, with statistically significant improvements (p-value < 0.001, Wilcoxon signed-rank test~\cite{wilcoxon1992individual}), while maintaining competitive inference efficiency.

\textbf{Effectiveness Analysis.} De-Hallucinator shows no improvement or even slight degradation compared to the base model. RAG achieves an EM of 35.45\%, but its high hallucination rate of 60.90\% on PanguCoder-11B limits its effectiveness. In contrast, {\tool} delivers significant improvements across all metrics. On PanguCoder-11B, it boosts EM by 71.79\%, ES by 31.52\%, and reduces MaHR by 58.21\% and MiHN by 57.53\% compared to RAG. These results demonstrate that merely providing relevant code snippets or iterative grounding is insufficient for industrial scenarios, while {\tool} effectively addresses these challenges by integrating project-specific dependencies and constrained decoding.

% De-Hallucinator performs worse, showing no improvement or even slight degradation compared to the base model. RAG achieves an EM of 35.45\% but suffers from a high hallucination rate of 60.90\% on PanguCoder-11B. In contrast, {\tool} achieves substantial gains across all metrics. For example, on PanguCoder-11B, it improves EM by 71.79\%, ES by 31.52\%; and reduces MaHR by 58.21\%, MiHN by 57.53\% compared to the best baseline, RAG. These results highlight that simply providing relevant code snippets or applying iterative grounding is insufficient for industrial scenarios while {\tool} can xxx. 
% This indicates that {\tool} can effectively mitigate the API hallucination in the industrial scenario by providing structural project context and constraining the decoding process.
% These results highlight that simply providing relevant code snippets or applying iterative grounding is insufficient for industrial scenarios while {\tool} can xxx. 

\textbf{Efficiency Analysis.} RAG and De-Hallucinator introduce substantial latency (e.g., 0.411s and 0.479s per sample on PanguCoder-11B) due to their reliance on retrieval and iterative processes. {\tool} achieves impressive efficiency, requiring only 0.235s per sample on PanguCoder-11B and 0.237s on PanguCoder-34B, adding just 0.030s and 0.033s overhead compared to base models. These results show that {\tool} is both effective and practical for industrial deployment, balancing performance with efficiency.
% \vspace{-2mm}
\begin{tcolorbox}[breakable,width=\linewidth-2pt,boxrule=0pt,top=2pt, bottom=2pt, left=4pt,right=4pt, colback=gray!15,colframe=gray!15]

\textbf{Answer to RQ4:} {\tool} demonstrates strong performance in industrial scenarios, achieving substantial improvements in both generation accuracy and hallucination mitigation while maintaining high efficiency.

\end{tcolorbox}
% \vspace{-2mm}

==> FSE25-Industry-APIMitigation_2/sections/6_discussion.tex <==
\begin{figure*}[t]
\setlength{\abovecaptionskip}{-1pt}
    \centering
   \subfigure[Different project contexts provided in the input prompt]{
        \centering
        \includegraphics[scale=0.45]{figures/case_1.pdf} 
        \label{fig:case_1}
    }
    \subfigure[Generation process with Top-3 token logits]{
        \centering
        \includegraphics[scale=0.45]{figures/case_2.pdf}
        \label{fig:case_2}
    }
    \caption{Case study on API hallucination mitigation across Base, De-Hallucinator, RAG, and {\tool} using CodeLlama-7B.}
    \label{fig:case}
\end{figure*}


% \subsection{Case Study}

% As shown in Figure~\ref{fig:case}, we revisit the example from the Introduction, where the {\tt update} function requires an API to determine an agent’s reaction to an observation.  
% % Let us continue with the example from the Introduction, the {\tt update} function requires accurate API generation to determine the agent's reaction to an observation. 
% There are six valid APIs for {\tt API\_Position}, including {\tt getCurrentActivity()}, {\tt getEmoji()}, 
% \\
% {\tt setEmoji(String)}, {\tt setReact(boolean)}, {\tt willReact()} and  
% \\
% {\tt setCurrentActivity(String).}
% % These results show how {\tool} integrates project context and decoding constraints to ensure accurate API generation and avoid hallucinations.
% % Figure~\ref{fig:case} demonstrates how {\tool} mitigates API hallucination through hierarchical dependency mining and constrained decoding, compared with Base, De-Hallucinator, and RAG.


% Figure~\ref{fig:case_1} illustrates the input context for each approach. The Base model relies solely on the incomplete function, generating the hallucinated API {\tt isReacting()}. De-Hallucinator provides relevant APIs but fails to link them to the function, producing the incorrect {\tt getReaction()}. RAG retrieves similar code snippets but neglects project-specific dependencies, leading to the invalid {\tt getReact()}. In contrast, {\tool} incorporates structured project context, such as {\tt Class World}'s skeleton and the implementation of called function {\tt getReaction}. This enriched input enables the model to leverage both local and global dependencies, providing a comprehensive context for the incomplete function, which allows it to accurately generate {\tt willReact()} while effectively suppressing invalid alternatives. Figure~\ref{fig:case_2} shows the token logits for each approach, revealing differences in generation confidence. The Base model shows high uncertainty with weak logits for its first token {\tt is} (-1.16). De-Hallucinator improves slightly, with stronger logits for {\tt get} (-1.06), and RAG retrieves broader context, resulting in logits of -0.88 for {\tt get} and -0.01 for {\tt act}. In contrast, {\tool}, through dependency constrained decoding, assigns a near-certain logit to {\tt will} (-0.01) at the first position, followed by deterministic logits for {\tt Re} (-4.8E-07) and {\tt act} (-3.6E-07), guided by the API prefix tree. The final {\tt ())} token is accurately predicted using parameter validation.


\subsection{Why does {\tool} work?}

The effectiveness of {\tool} lies in enriching the input context with structural project information and adaptively guiding the decoding process to adhere to valid APIs. As demonstrated in Figure~\ref{fig:case}, we revisit the example from the Introduction, where the {\tt update} function requires an API to determine an agent’s reaction to an observation. 

\subsubsection{Hierarchical dependency mining for enriching the input context with structural project information}

As shown in Figure~\ref{fig:case_1}, baseline approaches fail to provide sufficient context. The Base model relies solely on the incomplete function and generates the hallucinated API {\tt isReacting())}. De-Hallucinator retrieves relevant APIs but does not establish their connection to the function, producing the incorrect {\tt getReaction()}. Similarly, RAG retrieves similar code snippets but overlooks project-specific dependencies, leading to the invalid {\tt getReact())}. In contrast, {\tool} mines both local and global dependencies from the project such as the skeleton of {\tt Class World} and the implementation of {\tt getReaction} to create a structured and enriched input prompt. By providing a more comprehensive view of the project, {\tool} enables the model to accurately generate the API {\tt willReact())} while avoiding invalid alternatives.

\subsubsection{Dependency constrained decoding for adaptively guiding the generation process to valid API tokens.}

Figure~\ref{fig:case_2} shows the token logits for each approach, revealing differences in generation confidence. The Base model shows high uncertainty, with weak logits for its first token {\tt is} (-1.16). De-Hallucinator improves slightly, with stronger logits for {\tt get} (-1.06), and RAG retrieves broader context, resulting in logits of -0.88 for {\tt get} and -0.01 for {\tt act}. In contrast, {\tool} demonstrates near-certain logits for the correct token sequence, assigning -0.01 for {\tt will}, followed by deterministic logits for {\tt Re} (-4.8E-07) and {\tt act} (-3.6E-07). This precision is guided by the API prefix tree, ensuring that the generated tokens align with the project's valid APIs. Additionally, the final {\tt ())} token is accurately predicted through parameter validation, further enhancing the reliability of the generated code. By adaptively guiding the generation process, {\tool} ensures the generation complies with API specifications in the project, thus mitigating the API hallucination.

\subsection{Threats to Validity}

We identify four main threats to the validity of our study:

\textbf{Model Selection.} Although we have evaluated {\tool} on multiple models, including CodeLlama, DeepSeekCoder, and PanguCoder, many other LLMs remain unexplored, such as CodeQwen~\cite{codeqwen}, CodeGen~\cite{CodeGen}. However, the consistent improvements across current models suggest that our framework is highly generalizable. In the future, we will extend our evaluation to a wider range of models to further validate its scalability.

\textbf{Evaluation Tasks.} Our current implementation and evaluation are centered on Java projects. However, the design of {\tool} is language-agnostic, and we believe the framework can be extended to other programming languages with minimal adaptation, leveraging their respective dependency analysis.

\textbf{Prompt Design.} The effectiveness of {\tool} partially depends on our prompt template design. While we have conducted extensive experiments to validate our template, there might be room for further optimization. To mitigate this threat, we have open-sourced our prompt templates to facilitate community feedback and improvements. 

\textbf{Benchmark Curation.} Our benchmarks are created automatically. While automation enables scalability to handle extensive benchmarking tasks, it introduces potential concerns regarding dataset correctness and quality. In the future, we will enhance benchmark reliability by incorporating more extensive human validation or adopting hybrid dataset creation strategies.


% Figure 7 presents a case study on API hallucination mitigation across different approaches. For this update function in the reaction-checking context, the valid API should be willReact() based on the project's structural dependencies. However, we observe that Base, De-Hallucinator, and RAG all generate invalid APIs (isReacting(), getReaction(), and getReact() respectively), despite having different levels of context information.

% Analysis of the token-level logits in Figure 7(b) reveals varying degrees of generation confidence:

% Base model shows high uncertainty with weak logits for its first token "is" (-1.16) and subsequent tokens
% De-Hallucinator exhibits moderate confidence with slightly stronger logits for "get" (-1.06)
% RAG demonstrates higher but misplaced confidence with "get" (-0.88) and "act" (-0.01)
% These confidence patterns reflect the varying richness of project context provided to each method, as shown in Figure 7(a). While richer context does lead to more concentrated probability distributions, it still fails to prevent API hallucination without proper structural guidance.

% In contrast, our method leverages project-specific structural constraints through the API prefix tree and parameter patterns. The logits show strong confidence in selecting "will" (-0.01) as the first token, followed by near-deterministic selection of "Re" (-4.8E-07) and "act" (-3.6E-07) due to the prefix tree guidance. The final "()" token is correctly determined through our parameter pattern constraint. This demonstrates how our dependency-constrained decoding effectively prevents hallucination by combining both API structural knowledge and parameter validation.



==> FSE25-Industry-APIMitigation_2/sections/7_relatedWork.tex <==
\subsection{LLMs for Code Generation}

The impressive capabilities of LLMs in natural language processing have inspired researchers and companies to develop specialized models for code generation~\cite{CodeX,codellama,incoder,CodeGen,wavecoder,WizardCoder,mftcoder}. OpenAI proposes Codex~\cite{CodeX}, the earlier representative work of code LLMs. Subsequently, various models have emerged, such as Meta's InCoder~\cite{incoder} and CodeLlama~\cite{codellama}, Salesforce's CodeGen~\cite{CodeGen}, BigCode project's StarCoder series~\cite{starcoder,StarCoder2}, and Deepseek AI's DeepseekCoder~\cite{deepseek}. These code LLMs typically follow two development approaches: continuously training existing general models (e.g. CodeLlama), or training from scratch with code-specific data (e.g. DeepseekCoder). These advances have enabled commercial programming assistants like GitHub Copilot~\cite{copit} and Amazon CodeWhisperer~\cite{codewhisperer} demonstrate promising results in software development. Our proposed framework {\tool} can be applied seamlessly to current intelligent programming assistants to mitigate hallucinations in code generation, enhancing their accuracy and reliability.

\subsection{Hallucinations in LLMs}

While LLMs have shown remarkable performance in text generation, they frequently produce outputs that sound plausible but are incorrect, known as ``Hallucination'', severely impacting reliability and practical applications~\cite{text-1,text-2,relatedwork_hal1,relatedwork_hal2,relatedwork_hal3,relatedwork_hal4}. In the domain of code generation, hallucination poses similar challenges, particularly in scenarios involving API usage, where models may generate invalid API calls or misuse existing APIs. Liu~\textit{et al.}~\cite{liu2024exploring} conduct pioneering work in categorizing different types of code hallucinations. Zhang~\textit{et al.}~\cite{zhang2024llm} further explore the prevalence of code hallucinations in industrial settings, highlighting the unique challenges faced in real-world applications. Agarwal~\textit{et al.}~\cite{tian2024codehalu} propose a benchmark for detecting hallucinated code snippets on Python. To mitigate hallucination issues, Zhang~\textit{et al.}~\cite{zhang2024llm} retrieve project-specific code snippets to enhance generation. Eghbali \textit{et al.}~\cite{eghbali2024hallucinator} propose De-Hallucinator, which adds API references related to the model's predictions into the prompt. Jain \textit{et al.}~\cite{jain2024mitigating} introduce Documentation Augmented Generation (DAG), using API documentation from services like AWS and Azure to guide generation. Different from these approaches, our {\tool} combines project-specific structural context and dependency constrained decoding to ensure valid API generation, effectively mitigating hallucination in practical code generation scenarios.


% We demonstrate that Documentation Augmented Generation (DAG) significantly improves performance

% everal mitigation approaches have been proposed, including retrieval-based methods


% benchmark containing generated hallucinated code snippets for Python programming problems.

% developed metrics for measuring hallucination severity in generated code.


% , particularly in API usage scenarios where models may generate invalid API calls or misuse existing APIs. 

% Liu et al. [x] conducted pioneering work in categorizing different types of code hallucinations and their impact on code quality. Wang et al. [x] further analyzed the prevalence of API hallucinations in industrial settings, while Vibhor Agarwal et al. [x] developed metrics for measuring hallucination severity in generated code. Several mitigation approaches have been proposed, including retrieval-based methods [x], verification frameworks [x], and constrained generation techniques [x]. Our work extends this line of research by systematically studying API hallucination patterns and proposing a structural-aware solution that fundamentally addresses this challenge.


% Hallucination, where models generate factually incorrect or non-existent content, remains a significant challenge in LLMs. In code generation, this issue manifests primarily through API misuse and invalid references. Prior work has explored various aspects of this problem:

% \begin{itemize}

% \item \textit{Hallucination Classification}: Liu et al. [x] categorized different types of code hallucination; Wang et al. [x] analyzed their impact on code quality; Agarwal et al. [x] studied patterns of API misuse.

% \item \textit{Mitigation Approaches}: Several solutions have been proposed, including retrieval-augmented generation [x], post-generation validation [x], and constrained decoding [x].

% \end{itemize}

% Our work advances this field by systematically studying API hallucination in code generation, identifying different types of API misuse patterns, and proposing a novel structural-aware approach for mitigation. Unlike previous work that mainly focuses on post-processing or retrieval enhancement, MARIN integrates structural information during the generation process, leading to more reliable API usage.

% Hallucinates in LLMs
% Although LLMs have shown remarkable performance in natural language generation, they still inevitably encounter several issues, hallucination being one of the top. [具体幻觉是什么，影响是什么]. Similar to text hallucinations, LLMs can hallucinate during code generation as well. [ 对幻觉分类的部分 ]Liuxxx干了啥，Wangxx干了啥，Vibhor Agarwal干了啥。一些工作提出了【缓解方法】，xxx干了啥，xxx干了啥，xxx干了啥。In this work，我们系统性的研究了代码生成中的API幻觉问题，identify the differern。


% LLMs for code generation. 
% [LLM在自然语言xx上的impressive capability has inspired researchers and companies to develop specifd LLMs for code generation。这些模型有两种训练方式，continuously training foundation LLMs or directly training from scratch。，such as xxx，xxx，xxx，xxx，xxx。基于这些模型，许多公司开发了智能编程助手，如copilt，wisper，xxx。这些智能编程助手xxxx。我们的方法通过对xxx and logits and hence can be used with any model.

% \textbf{Hallucination in Language Models.}

% Although LLMs have shown remarkable performance in natural language generation, they still inevitably suffer from hallucination - generating content that is factually incorrect or inconsistent with given context. Such hallucinations can manifest as fabricated facts, contradictory statements, or non-existent references, severely impacting model reliability and practical applications. In code generation, similar hallucination issues persist, particularly in API usage scenarios where models may generate invalid API calls or misuse existing APIs. Liu et al. [x] conducted pioneering work in categorizing different types of code hallucinations and their impact on code quality. Wang et al. [x] further analyzed the prevalence of API hallucinations in industrial settings, while Vibhor Agarwal et al. [x] developed metrics for measuring hallucination severity in generated code. Several mitigation approaches have been proposed, including retrieval-based methods [x], verification frameworks [x], and constrained generation techniques [x]. Our work extends this line of research by systematically studying API hallucination patterns and proposing a structural-aware solution that fundamentally addresses this challenge.


==> FSE25-Industry-APIMitigation_2/sections/8_conclusion.tex <==
In this paper, we propose
% proposed 
{\tool}, a framework designed to mitigate API hallucination based on hierarchical dependency analysis. By identifying local and global dependencies in the incomplete function and applying dependency constrained decoding, {\tool} ensures the generated APIs align with project requirements. Experiments show that {\tool} significantly improves API accuracy, reduces hallucination rates, and maintains efficiency with minimal overhead. In addition, {\tool}’s strong performance in industrial scenarios demonstrates its effectiveness in generating accurate and reliable APIs. As a solution to mitigate API hallucination in LLM-driven code generation, {\tool} contributes to the development of accurate and reliable code generation systems. In future work, we plan to extend {\tool} to a wider range of LLMs, additional programming languages, and optimize our prompt template.



==> FSE25-Industry-APIMitigation_2/todo.tex <==
1) abs:
2) intro
Figure1: 三种API幻觉场景
3) preliminary 【三个模型】codellama 7b 13b 34b
Figure2 (a)(b): 两种类型的API都是啥样的 / 三种场景是什么
Figure2 (c)(d): 不同api的结果 / 不同context的结果
4）approach
figure3 framework
figure4 prompt是啥样的
figure5 前缀树
Text Refine 
5）setup
Text：inference details需要加上
6）result
RQ1. Table填写完整 / 实验分析 / 
RQ2. Figure调整好 / 实验分析 / 
RQ3. Table填写完整 / 实验分析 / 
RQ4. Table调整好 / 实验分析 / 
7）discussion
进行case study 
1) project context 有用
2）干预有用 （project context仍然不能正确回答）
对应找两个例子



Something needs discussion
1) 是否需要双盲？
1) generate what
2) 需要对什么生成有准确的定义 , 比如说都叫 focal function
3) 


pre exp
1. API type （幻觉率）
Codellama 7B
third ： 0.1454
project：0.8272
Codellama 13B
third ：0.1090
project： 0.8454
DSC 1.3B
third ：0.1272
project： 0.8727
DSC 6.7B
third ：0.1181
project： 0.8636

2. Input Context （幻觉率）
Codellama 7B
base 0.8272
rag  0.7272
project  0.6521
api 0.5636

Codellama 13B
base  0.8454
rag  0.7181
project 0.6884
api  0.5289

DSC 1.3B
base  0.8727
rag  0.7181
project  0.6959
api  0.5818

DSC 6.7B
base 0.8636
rag 0.7727
project 0.6884
api  0.5727

aba exp

API-F

codellama 7b

EM
base -/+干预  21.71 / 28.05
base + local  -/+干预  41.17  / 46.15
base + Global  -/+干预  51.58 / 58.37
base + local + Global -/+干预 66.96  / 76.01

MaHR
base -/+干预   73.30  / 59.72
base + local  -/+干预 55.20 / 47.05
base + Global  -/+干预  38.91 / 31.67
base + local + Global -/+干预 27.14 / 15.83


codellama 13b

EM
base -/+干预  33.03 / 4072
base + local  -/+干预 49.32 / 53.39
base + Global  -/+干预  55.20 / 62.89
base + local + Global -/+干预 60.63  /66.96


MaHR
base -/+干预  61.08 / 49.32
base + local  -/+干预  46.60 / 40.27
base + Global  -/+干预  35.29 / 27.14
base + local + Global -/+干预 32.57 / 15.83


codellama 34b

EM
base -/+干预  19.45 / 25.79
base + local  -/+干预 34.38 / 38.91
base + Global  -/+干预  53.84 / 58.37
base + local + Global -/+干预 69.23 / 81.90

MaHR
base -/+干预   75.56 / 65.61
base + local  -/+干预 61.99 / 53.84
base + Global  -/+干预  38.00 / 33.03
base + local + Global -/+干预 24.88 / 12.66


ds 1.3b

EM
base -/+干预   20.81 / 39.81
base + local  -/+干预 44.79 / 51.58
base + Global  -/+干预  56.56 / 64.25 
base + local + Global -/+干预 65.61 / 75.11


MaHR
base -/+干预   75.56 / 45.24
base + local  -/+干预 51.13 / 39.36
base + Global  -/+干预  36.19 / 28.05
base + local + Global -/+干预 27.60 / 17.64 

ds 6.7b

EM
base -/+干预   20.81 / 27.60
base + local  -/+干预 48.41 / 52.94
base + Global  -/+干预  59.27 / 68.32
base + local + Global -/+干预 68.77 / 75.56 


MaHR
base -/+干预  75.56  / 58.37
base + local  -/+干预 47.05 / 39.36
base + Global  -/+干预  29.86 / 20.36
base + local + Global -/+干预 24.43 / 16.74


ds 33b

EM
base -/+干预   35.74 / 40.72
base + local  -/+干预 57.91 / 59.72
base + Global  -/+干预  61.53 / 71.49 
base + local + Global -/+干预 71.49 / 81.90


MaHR
base -/+干预   59.72 / 45.70
base + local  -/+干预  38.46 / 33.03
base + Global  -/+干预    31.22   / 20.81
base + local + Global -/+干预  23.07 / 11.76


API-M

codellama 7b

EM
base -/+干预  27.69/ 42.05
base + local  -/+干预 31.79 / 35.89
base + Global  -/+干预  48.20 / 56.41
base + local + Global -/+干预 56.41 / 66.66


MaHR
base -/+干预   65.12 / 40.51
base + local  -/+干预 56.92 / 44.61
base + Global  -/+干预  30.25 / 21.53
base + local + Global -/+干预  23.07 / 12.30 


codellama 13b

EM
base + /- 干预   33.33 / 40.51
base + local  -/+干预 37.43 / 43.58
base + Global  -/+干预   46.15 / 57,94
base + local + Global -/+干预  55.89 / 66.66 


MaHR
base -/+干预   59.48 / 40.51
base + local  -/+干预 49.23 / 38.46
base + Global  -/+干预  31.79 /  0.20
base + local + Global -/+干预 24.10 / 12.30 


codellama 34b

EM
base -/+干预   24.61 / 34.35
base + local  -/+干预 32.30 / 37.43
base + Global  -/+干预  49.23 / 61.53
base + local + Global -/+干预 59.48 / 70.76


MaHR
base -/+干预   68.71 / 48.20
base + local  -/+干预 56.41 / 43.07
base + Global  -/+干预  30.25 / 17.94
base + local + Global -/+干预 22.56 / 10.76


ds 1.3b

EM
base -/+干预   23.58 / 32.30
base + local  -/+干预 38.46 / 40.51
base + Global  -/+干预  40.00 / 52.30
base + local + Global -/+干预 52.30 / 64.61


MaHR
base -/+干预   68.20 / 49.23
base + local  -/+干预 51.28/ 41.02
base + Global  -/+干预  37.94 / 26.15
base + local + Global -/+干预 27.69 / 15.38 


ds 6.7b

EM
base -/+干预   23.07 / 33.33
base + local  -/+干预 35.89 / 43.07
base + Global  -/+干预  49.74 / 64.10
base + local + Global -/+干预 56.92 / 68.20


MaHR
base -/+干预   68.71 / 48.71
base + local  -/+干预 52.82 / 40.00
base + Global  -/+干预  29.74 / 15.38
base + local + Global -/+干预 23.07/11.28


ds 33b

EM
base -/+干预   20.00 / 28.20
base + local  -/+干预 40.51 / 56.92
base + Global  -/+干预  50.25 / 63.58
base + local + Global -/+干预 55.89/ 67.69


MaHR
base -/+干预   70.25 / 50.76
base + local  -/+干预 43.58 / 22.56
base + Global  -/+干预  27.69 / 14.35
base + local + Global -/+干预 24.61/ 9.74 

{'model': '/home/workspace/jiangzhihan/PanguDevL1.13-sharding', 'prompt': '\n// Here are some potential APIs.\n// public String getFullTimeFormat() \n// public String getTimeFormat() \n// public String getApiPath() \n@Override\n    public boolean update(IChatService service, World world, Agent agent) {\n\tLOG.info("[Updater / Reaction] Checking if an agent will react to an observation");\n\n\tReaction reaction = service.getReaction(agent, observation);\n\n\tif (reaction.', 'max_tokens': 15, 'temperature': 0, 'stream:': True, 'oracle_str_book': None, 'gold': 'willReact()', 'index': 22}

194 221

110

==> datas/benchmark-statistics.tex <==
\begin{table}[]
\centering
\begin{tabular}{lrrrr}
\toprule
\textbf{Benchmark}                 & \textbf{APIHulBench} \\
\midrule
\ Language                        & Java             \\
\# Repositories                  & 244             \\
\# Files                         & 47751           \\
\# Examples                      & 2856           \\
Avg. \# lines in prompt          & 18.34          \\
Avg. \# tokens in prompt         & 145.73           \\
Avg. \# lines in reference       & 1.0             \\
Avg. \# tokens in reference      & 8.18            \\
\bottomrule
\end{tabular}
\caption{APIHulBench statistics.}
\label{tab:crosscodeeval}
\end{table}


==> sections/2_preStudy.tex <==
% API hallucination, in which large language models (LLMs) incorrectly generate API-related code, has become a critical challenge in software engineering tasks. To evaluate and analyze this phenomenon, several benchmarks have been introduced. For example, the recently proposed CrossCodeEval~\cite{ding_crosscodeeval_2023} focuses primarily on cross-file code completion, but ignores the widespread reliance on third-party libraries in real-world software development. CloudAPIBench~\cite{jain_mitigating_2024} explores the use of third-party APIs. However, it does not incorporate project-specific APIs, lacking a comprehensive evaluation of project-level contextual dependencies.

% Given that both API type and API call frequency significantly influence model performance, we propose APIHulBench, a benchmark designed to evaluate API hallucination across varying frequencies (high-frequency and low-frequency APIs) and types (third-party and project-specific APIs). By conducting extensive evaluations on multiple state-of-the-art LLMs, our work provides an in-depth analysis of how different API characteristics impact hallucination. We reveal key sources of confusion that contribute to API hallucinations and provide targeted insights for subsequent research on mitigating API hallucinations.


\modify{While previous studies have identified the phenomenon of API hallucination in LLMs~\cite{}, there is still a lack of comprehensive studies exploring its characteristics and mitigation strategies. To fill this gap, we introduce {\dataset}, a comprehensive benchmark for evaluating real-world API hallucinations. We then evaluate four representative LLMs on {\dataset} to investigate hallucination patterns across various API types, offering valuable insights for developing effective mitigation strategies.}
 
\subsection{{\dataset}} \label{sec:benchmark}

% 

\subsubsection{Benchmark Construction }

\textit{Dataset Collection.}

\textit{API Type Annotations.}

\textit{API Frequency Annotations.}


\subsubsection{Format and Statistics}


\textit{Data Format.}


\textit{Data Statistics.} As a result, we obtain xxxx. 

In this section, we aim to 

briefly describe how we collect software repositories, select a subset of them for the {\dataset} construction, classify the APIs called from the selected repositories in terms of type and frequency, and APIHulBench statistics. The APIHulBench construction process is illustrated in ~\ref{fig:benchmark}. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/benchmark.png}
    \caption{The APIHulBench construction process.}
    \label{fig:benchmark}
\end{figure}

\textbf{Dataset Collection.} We 

collected over 99 stars of Java repositories from GitHub and then filtered out repositories with code files larger than 1,000, ending up with 10,605 repositories. These repositories will be used for third-party API call frequency statistics. In general, when building benchmarks for code LLMs, it is essential to reduce data leakage, i.e., we must ensure that the data in the benchmarks are not trained by the models. Therefore, we focus on recently created repositories. Specifically, we filtered out repositories created after 2023 from the 10,605 repositories collected, totaling 244 repositories. This ensures that the amount of data collected is large enough and does not overlap with the training data of many existing large code models released before 2023, avoiding underestimation of the API hallucination rate.


\textbf{API Type Annotations.} In order to distinguish the external knowledge required by different types of APIs, we classify API calls into two categories: project-specific APIs and third-party APIs. First,we parse each file in the repository and extract file-level imported libraries. The imported libraries are usually explicitly declared through import statements and reflect the classes and libraries the current file depends on. Next, based on the path information of the imported libraries, they match the file structure of the repository. If the path to an imported library can be found in the current project's directory, the imported library is considered an internal library, and it is inferred that the API call belongs to a project-specific API; otherwise, if the path to the imported library is not in the project's repository, but comes from an external dependency (e.g., the Java Standard Library, third-party libraries, or frameworks), the imported library is labeled as an external library, and the associated API call is classified as a third-party APIs.


\textbf{API Frequency Annotations.} In order to explore whether there is a difference in the hallucination rate of APIs with different frequencies in LLMs/LCMs, APIHubBench further categorises the frequency of API usage. Based on the classification of API types, we statistically analysed the frequency of third-party API calls using data collected from 10,605 code repositories. Due to the sufficiently large size of the data, these 10,605 code repositories can be considered as a reasonable approximation of the distribution of real-world APIs. Therefore, we can use them to explore the relationship between the hallucination rate of various code LLMs and the API frequency. Specifically, we filtered 244 target repositories from 10,605 code repositories and counted the frequency of third-party API calls in these repositories. Subsequently, based on the number of occurrences of APIs in the 10,605 repositories, we classify APIs into two categories: low-frequency APIs (\(\leq 10\) invocations) and high-frequency APIs (\(\geq 100\) invocations). This classification method follows the idea of grouping concepts by their popularity or frequency in pre-trained data~\cite{mallen_when_2023}~\cite{razeghi_impact_2022}.

\input{datas/benchmark-statistics}

\textbf{Construction.} Our purpose of constructing the APIHulBench was to extend the classification on the API hallucination. Thus we classified APIs into project- specificed kinds and third-party kinds, and among third-party APIs we further classified them into high-frequency and low-freqwuency APIs, which eventually yielded 1073 project- specificed APIs, 1603 third-party high-frequency APIs and 139 third-party low-frequency APIs, respectively. The statistics of APIHulBench are presented in table1(). For each api data, we add three levels of information, repo-level, file-level and function-level.Specific information on the three levels is as follows:
\begin{itemize}
\item {\textbf{Repo-level information}} includes the name of the repository, an overall description of the repository, and the external libraries or frameworks that the repository depends on.
\item {\textbf{File-level information}} includes import information in the file, class, function, and variable definitions defined in the file, and comments in the header or significant parts of the file.
\item {\textbf{Function-level information}} includes the name of the function, the name of the class to which it belongs, the signature of the function, the function's documentation string, the function's parameters and their types, the context of the function's code fragment, information about the target API called in the function, other internal methods called by the function, and external libraries called in the function.
\end{itemize}

\subsection{Studied Baselines} \label{sec:preStudy baseline}
\quad In order to initially evaluate the performance of the model on different types and frequencies of APIs, we extracted part of the data from APIHulBench, and the extraction process prioritized the diversity of the data to ensure that the data on the same category came from different repositories, and finally extracted 131 project-specified API data, 179 third-party high-frequency API data and 161 third-party low-frequency API data. As shown in Table(), we selected four representative LLMs (Llama-7B~\cite{}, Deepseek-33B~\cite{}, StarCoder2-15b~\cite{}, GPT-4~\cite{}) for evaluation. These four models cover a wide range of sizes and training objectives, from small to large models, and encompass state-of-the-art large code modelling techniques. 

\subsection{Metrics} \label{sec:metrics}
\quad In our preliminary study on exploring the performance of different types and frequencies of APIs in LLM, we mainly used \textbf{Exact Match (EM)}, \textbf{Editorial Similarity (ES)} and \textbf{Identifier Matching} as evaluation metrics. Taking into account elements such as identifiers, keywords, operators and delimiters, the EM and ES metrics help evaluate the overall accuracy of the code completion process. The identifier matching metric evaluates the ability of the model to generate the correct Application Programming Interface (API). For the evaluation, we parse the code and extracted identifiers from model generations, which are compared against the ground-truth identifiers to compute the F1 score.

Additionally, to quantify a Code LLM's uncertainty during API invocation, we define \textbf{API invocation confidence} as the minimum probability among all predicted API name tokens.~\cite{} Because the API name represents the core function or operation being invoked and has a large impact on subsequent reasoning, we focus only on the invocation confidence of the API name.

Furthermore, based on the correctness of the API calls, we classify the results into four types to more precisely analyze the sources of confusion in the model~\cite{}:

\textbf{Type 1: Completely Correct. }This type indicates that the model accurately generated both the correct API name and parameters, resulting in a fully correct API call.

\textbf{Type 2: API Name Correct.} Parameters Incorrect: This type indicates that the model successfully predicted the correct API name but made errors in the parameters. 

\textbf{Type 3: Incorrect but Existing API Called. }This type indicates that the model selected an incorrect API, even though the API exists in an external library or the project. 

\textbf{Type 4: Non-existent API Called.} THis type can be caused by two reasons,  either the API does not exist in the repository, or the API is not available in the external library that the model is calling. It reflects the model's lack of knowledge or misunderstanding of the external library.


\subsection{Results} \label{sec:result}

\quad Table 1() shows the performance of the model on different types and frequencies of APIs. Based on the experimental results, we derive the following findings:



Analysing this xx, we obxxx. 

\textbf{Observation 1.} [xxx]

\textbf{Observation 2.} [xxx]

Therefore, in this work, we propose to xxx.

\textbf{API type and frequency have a significant impact on the generation of model hallucinations.} Regarding API frequency, we observe a strong correlation between API frequency and effective API calls. On the other hand, in terms of API type, project-specific APIs are much more likely to hallucinate than high-frequency third-party APIs, but only slightly more likely than low-frequency third-party APIs. This suggests that the model lacks sufficient training data for low-frequency APIs, and lacks sufficient contextual knowledge for project-specific APIs, both of which tend to have higher hallucination rates.

\textbf{There is a strong correlation between API call accuracy and API call confidence.} Experiments have shown that the accuracy rate of API calls tends to be positively correlated with the API call confidence when the model predicts API names. When the model has higher API call prediction confidence, call accuracy is correspondingly higher. This finding indicates that API Invocation Confidence can be an important indicator of a model's prediction reliability.

\textbf{There are differences in the knowledge required for different types of APIs.} For third-party APIs, the main source of confusion for the model comes from ``calling the wrong but existing API'' (Type 3). This type of error is usually due to the model choosing a semantically or syntactically valid API in an external library or framework that is not applicable in the current context, reflecting the model's limited understanding of the external knowledge. For project-specific APIs, the model's main confusion stems from “calling an API that does not exist” (Type 4). This type of error may be due to the lack of accurate modeling of the project context in the model for project-specific APIs, resulting in the generated API names not matching the actual project. This further suggests that the model requires richer project-level contextual information and customization knowledge when dealing with project-specific APIs. This difference further reveals the different emphasis of the two types of APIs on relying on knowledge and contextual information external to the model.


==> todo.tex <==
1) abs:
2) intro
Figure1: 三种API幻觉场景
3) preliminary 【三个模型】codellama 7b 13b 34b
Figure2 (a)(b): 两种类型的API都是啥样的 / 三种场景是什么
Figure2 (c)(d): 不同api的结果 / 不同context的结果
4）approach
figure3 framework
figure4 prompt是啥样的
figure5 前缀树
Text Refine 
5）setup
Text：inference details需要加上
6）result
RQ1. Table填写完整 / 实验分析 / 
RQ2. Figure调整好 / 实验分析 / 
RQ3. Table填写完整 / 实验分析 / 
RQ4. Table调整好 / 实验分析 / 
7）discussion
进行case study 
1) project context 有用
2）干预有用 （project context仍然不能正确回答）
对应找两个例子



Something needs discussion
1) 是否需要双盲？
1) generate what
2) 需要对什么生成有准确的定义 , 比如说都叫 focal function
3) 


pre exp
1. API type （幻觉率）
Codellama 7B
third ： 0.1454
project：0.8272
Codellama 13B
third ：0.1090
project： 0.8454
DSC 1.3B
third ：0.1272
project： 0.8727
DSC 6.7B
third ：0.1181
project： 0.8636

2. Input Context （幻觉率）
Codellama 7B
base 0.8272
rag  0.7272
project  0.6521
api 0.5636

Codellama 13B
base  0.8454
rag  0.7181
project 0.6884
api  0.5289

DSC 1.3B
base  0.8727
rag  0.7181
project  0.6959
api  0.5818

DSC 6.7B
base 0.8636
rag 0.7727
project 0.6884
api  0.5727

aba exp

API-F

codellama 7b

EM
base -/+干预  21.71 / 28.05
base + local  -/+干预  41.17  / 46.15
base + Global  -/+干预  51.58 / 58.37
base + local + Global -/+干预 66.96  / 76.01

MaHR
base -/+干预   73.30  / 59.72
base + local  -/+干预 55.20 / 47.05
base + Global  -/+干预  38.91 / 31.67
base + local + Global -/+干预 27.14 / 15.83


codellama 13b

EM
base -/+干预  33.03 / 4072
base + local  -/+干预 49.32 / 53.39
base + Global  -/+干预  55.20 / 62.89
base + local + Global -/+干预 60.63  /66.96


MaHR
base -/+干预  61.08 / 49.32
base + local  -/+干预  46.60 / 40.27
base + Global  -/+干预  35.29 / 27.14
base + local + Global -/+干预 32.57 / 15.83


codellama 34b

EM
base -/+干预  19.45 / 25.79
base + local  -/+干预 34.38 / 38.91
base + Global  -/+干预  53.84 / 58.37
base + local + Global -/+干预 69.23 / 81.90

MaHR
base -/+干预   75.56 / 65.61
base + local  -/+干预 61.99 / 53.84
base + Global  -/+干预  38.00 / 33.03
base + local + Global -/+干预 24.88 / 12.66


ds 1.3b

EM
base -/+干预   20.81 / 39.81
base + local  -/+干预 44.79 / 51.58
base + Global  -/+干预  56.56 / 64.25 
base + local + Global -/+干预 65.61 / 75.11


MaHR
base -/+干预   75.56 / 45.24
base + local  -/+干预 51.13 / 39.36
base + Global  -/+干预  36.19 / 28.05
base + local + Global -/+干预 27.60 / 17.64 

ds 6.7b

EM
base -/+干预   20.81 / 27.60
base + local  -/+干预 48.41 / 52.94
base + Global  -/+干预  59.27 / 68.32
base + local + Global -/+干预 68.77 / 75.56 


MaHR
base -/+干预  75.56  / 58.37
base + local  -/+干预 47.05 / 39.36
base + Global  -/+干预  29.86 / 20.36
base + local + Global -/+干预 24.43 / 16.74


ds 33b

EM
base -/+干预   35.74 / 40.72
base + local  -/+干预 57.91 / 59.72
base + Global  -/+干预  61.53 / 71.49 
base + local + Global -/+干预 71.49 / 81.90


MaHR
base -/+干预   59.72 / 45.70
base + local  -/+干预  38.46 / 33.03
base + Global  -/+干预    31.22   / 20.81
base + local + Global -/+干预  23.07 / 11.76


API-M

codellama 7b

EM
base -/+干预  27.69/ 42.05
base + local  -/+干预 31.79 / 35.89
base + Global  -/+干预  48.20 / 56.41
base + local + Global -/+干预 56.41 / 66.66


MaHR
base -/+干预   65.12 / 40.51
base + local  -/+干预 56.92 / 44.61
base + Global  -/+干预  30.25 / 21.53
base + local + Global -/+干预  23.07 / 12.30 


codellama 13b

EM
base + /- 干预   33.33 / 40.51
base + local  -/+干预 37.43 / 43.58
base + Global  -/+干预   46.15 / 57,94
base + local + Global -/+干预  55.89 / 66.66 


MaHR
base -/+干预   59.48 / 40.51
base + local  -/+干预 49.23 / 38.46
base + Global  -/+干预  31.79 /  0.20
base + local + Global -/+干预 24.10 / 12.30 


codellama 34b

EM
base -/+干预   24.61 / 34.35
base + local  -/+干预 32.30 / 37.43
base + Global  -/+干预  49.23 / 61.53
base + local + Global -/+干预 59.48 / 70.76


MaHR
base -/+干预   68.71 / 48.20
base + local  -/+干预 56.41 / 43.07
base + Global  -/+干预  30.25 / 17.94
base + local + Global -/+干预 22.56 / 10.76


ds 1.3b

EM
base -/+干预   23.58 / 32.30
base + local  -/+干预 38.46 / 40.51
base + Global  -/+干预  40.00 / 52.30
base + local + Global -/+干预 52.30 / 64.61


MaHR
base -/+干预   68.20 / 49.23
base + local  -/+干预 51.28/ 41.02
base + Global  -/+干预  37.94 / 26.15
base + local + Global -/+干预 27.69 / 15.38 


ds 6.7b

EM
base -/+干预   23.07 / 33.33
base + local  -/+干预 35.89 / 43.07
base + Global  -/+干预  49.74 / 64.10
base + local + Global -/+干预 56.92 / 68.20


MaHR
base -/+干预   68.71 / 48.71
base + local  -/+干预 52.82 / 40.00
base + Global  -/+干预  29.74 / 15.38
base + local + Global -/+干预 23.07/11.28


ds 33b

EM
base -/+干预   20.00 / 28.20
base + local  -/+干预 40.51 / 56.92
base + Global  -/+干预  50.25 / 63.58
base + local + Global -/+干预 55.89/ 67.69


MaHR
base -/+干预   70.25 / 50.76
base + local  -/+干预 43.58 / 22.56
base + Global  -/+干预  27.69 / 14.35
base + local + Global -/+干预 24.61/ 9.74 

{'model': '/home/workspace/jiangzhihan/PanguDevL1.13-sharding', 'prompt': '\n// Here are some potential APIs.\n// public String getFullTimeFormat() \n// public String getTimeFormat() \n// public String getApiPath() \n@Override\n    public boolean update(IChatService service, World world, Agent agent) {\n\tLOG.info("[Updater / Reaction] Checking if an agent will react to an observation");\n\n\tReaction reaction = service.getReaction(agent, observation);\n\n\tif (reaction.', 'max_tokens': 15, 'temperature': 0, 'stream:': True, 'oracle_str_book': None, 'gold': 'willReact()', 'index': 22}

194 221

110
